Learning Event-triggered Control from Data through Joint Optimization

We present a framework for model-free learning of event-triggered control strategies. Event-triggered methods aim to achieve high control performance while only closing the feedback loop when needed. This enables resource savings, e.g., network bandwidth if control commands are sent via communication networks, as in networked control systems. Event-triggered controllers consist of a communication policy, determining when to communicate, and a control policy, deciding what to communicate. It is essential to jointly optimize the two policies since individual optimization does not necessarily yield the overall optimal solution. To address this need for joint optimization, we propose a novel algorithm based on hierarchical reinforcement learning. The resulting algorithm is shown to accomplish high-performance control in line with resource savings and scales seamlessly to nonlinear and high-dimensional systems. The method's applicability to real-world scenarios is demonstrated through experiments on a six degrees of freedom real-time controlled manipulator. Further, we propose an approach towards evaluating the stability of the learned neural network policies.

==> chapters/5_ProofOfConceptChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TeX root = ../report.tex

\chapter{Proof of Concept}
\label{chp:ProofOfConcept}

In the following chapter, a proof of concept for the previously presented ideas and algorithms is presented. We apply the concepts to a slightly modified version of the OpenAI Gym Pendulum environment \cite{openaigym}.

\section{Parametrization of the proposed Algorithm}
\label{sec:parametrization}

Before proceeding, we first provide insights on how we implement the major components needed for the proposed algorithm (\algref{alg:learn_etc}). We use the same design choices for all the results presented from here on.

As explained in \secref{sec:leveragingrl_etc}, our implementation is based on three main components, the policy over options $\mu(o|\tilde{x})$, the intra option policy $\pi(u|\tilde{x},o)$, and the Q-function $Q(\tilde{x},u)$. \figref{fig:arch_pol_op}, \figref{fig:arch_intra_op}, and \figref{fig:arch_q_fct} show the standard implementations of the respective components for the case of using 2 options. \figref{fig:arch_intra_op} illustrates that for the case of performing the \gls{zoh}, \ie option 0, the intra option policy does not have to be evaluated. Thus, computational resources can be saved in the forward, as well as the backward pass. For implementing the \gls{nn} estimator of the Q-function (see \figref{fig:arch_q_fct}), we decided to split the estimates for option 0 and option 1 already before the first hidden layer. The reason for this choice is that as the two options are very different, we also expect very different Q-values for the two options, although being in the same state $\tilde{x}$. This is due to the fact that option 0 is limited to the \gls{zoh}, while option 1 can basically apply any action, depending on the intra option policy. For the same reasons, we arrive at the design choice for the policy over options (see \figref{fig:arch_pol_op}).

For the stability verification and retraining procedure, we apply the following modifications to the previously presented implementation. Instead of using the \gls{tanh} activation function, we apply the \gls{relu} activation. The number of hidden neurons is decreased from 64 to 32. This is due to the fact that at the core of the verification algorithm, we run a modified version of the Simplex algorithm, which simply runs faster if less neurons are used. Further, instead of using the softmax activation function for the policy over options, we calculate $Z=\zeta_0-\zeta_1$. If $Z>0$, this corresponds to performing the \gls{zoh} and choosing option 0, otherwise we use option 1. That way, we achieve deterministic behavior of the policy over options and avoid using the softmax activation function. Moreover, this deterministic decision is compatible with the stochastic case, as $Z=0$ equals to $\mu(o=0|\tilde{x})=\mu(o=1|\tilde{x})=\SI{50}{\percent}$, and $Z>0$ corresponds to $\mu(o=0|\tilde{x})>\mu(o=1|\tilde{x})$.

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/POC/NN/pol_op.png}
\caption{Exemplary illustration of the parametrization of the policy over options. In this specific implementation, each hidden layer consists of 64 neurons, and the \gls{tanh} and softmax activation functions are used. The variables $\zeta_0$ and $\zeta_1$ represent intermediate values.}
\label{fig:arch_pol_op}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/POC/NN/intra_opt.png}
\caption{Exemplary illustration of the parametrization of the intra option policy. In this specific implementation, each hidden layer consists of 64 neurons, and the \gls{tanh} activation function is used.}
\label{fig:arch_intra_op}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/POC/NN/q_fct.png}
\caption{Exemplary illustration of the parametrization of the Q-function estimator. In this specific implementation, each hidden layer consists of 64 neurons, and the \gls{tanh} activation function is used.}
\label{fig:arch_q_fct}
\end{figure}

\section{Introducing the Simulation Environment}

The equations of motion, in discrete-time, of the pendulum, are given by
\begin{equation}
\begin{split}
\theta[k+1] &= \theta[k] + \Delta T \dot{\theta}[k] + v_\theta[k]  \\
\dot{\theta}[k+1] &= \dot{\theta}[k] + \Delta T \ddot{\theta}[k] + v_{\dot{\theta}}[k]\\ 
&=\dot{\theta}[k] + \Delta T (\frac{-3g}{2l} \sin(\theta[k] + \pi ) + \frac{3}{ml^2} u[k]) + v_{\dot{\theta}}[k] \text{ ,}
\end{split}
\end{equation}

where $\theta$ represents the angle, $\dot{\theta}$ the angular velocity, $v$ the process noise, $u$ the control action, $\Delta T$ the time discretization, $m$ and $l$ the mass and the length of the pendulum, and $g$ the gravitational constant. The process noise is drawn from a standard normal distribution, scaled by $10^{-4}$. In addition, we add measurement noise $w$ of the same magnitude. Thus, the measurements are $\hat{\theta}[k]=\theta[k]+w_{\theta}[k]$, and $\hat{\dot{\theta}}[k]=\dot{\theta}[k]+w_{\dot{\theta}}[k]$. Those equations represent a forward integration of the nonlinear dynamics of the system in continuous time, and they do not include any damping.

If not stated differently, the goal is to stabilize the pendulum on top, \ie to keep the angle around $\theta=\SI{0}{\degree}$. When linearizing the original nonlinear, continuous-time, differential equation around this equilibrium, we arrive at $\ddot{\theta}=\frac{3g}{2l}\theta+\frac{3}{ml^2}u$. Using the values from the original environment, we get a time constant of the linearized system of $\tau=\sqrt{\frac{2l}{3g}} \approx \SI{0.26}{\second}$. 

Therefore, using a sampling rate of \SI{20}{\Hz}, as specified in the original implementation, should be sufficient for reliable and stable feedback control. This choice is rather on the lower end of the rule of thumb in feedback control that the sampling rate should be 5-10 times faster than the system dynamics. Thus, achieving huge communication savings is already a challenging problem.

\section{Learning Event-triggered Control}

In the following, we present results on learning \gls{et} control from scratch on the pendulum, using \algref{alg:learn_etc} and \eqref{eq:zoh_gen_opt}.

The control cost at each timestep is given by 
\begin{equation}
\label{eq:ctrl_cost}
J_{\text{ctrl}}[k]=1.0 \theta[k] + 0.1 \dot{\theta}[k] + 0.1 u[k] \text{ ,}
\end{equation}
and the overall cost is given by \eqref{eq:cost_fct}, using $\gamma=0.99$. The associated reward $R$ is obtained through $R=-J$. Those parameters are the same as in the standard OpenAI Gym implementation. We only increased the penalization on the control input from 0.001 to 0.1 to prevent the controller from being too aggressive.

\begin{figure}
\centering
\includegraphics[width=0.85\textwidth]{img/POC/stabilize/Learning_progress.png}
\caption{Illustration of the evolution of $R=-J$ during training, depending on the communication penalty $\lambda$. For higher values of $\lambda$, the final reward is bigger. It also seems that the higher $\lambda$, \ie the more resource-efficient one wants to be, the slower the training process.}
\label{fig:train_speed_top}
\end{figure}

\figref{fig:train_speed_top} illustrates the training progress for different values of the communication penalization factor $\lambda$. For higher values of $\lambda$, the overall reward $R$ is lower as the communication penalty is higher and increasing the communication savings negatively affects the control performance. Moreover, it also seems that the number of epochs it takes, until the training runs converge is larger for larger values of $\lambda$. This might reflect the fact that it is tougher to come up with a very resource-efficient control and communication strategy than with a policy that does not have to save as much communication due to a lower value of $\lambda$. While for $\lambda=0$, the average communication savings are around \SI{5}{\percent} (see \figref{fig:5percent_pend_top}), $\lambda=5.0$ results in communication savings up to around \SI{90}{\percent} (see \figref{fig:5percent_pend_top}). Those results are in line with the findings presented in \cite{BaumannRL}.

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/stabilize/eval_model_param-5_commpen5-0_seed200_exemplary_rollout_improved.eps}
	\caption{Illustration of the performance of a learned communication and control policy that saves about \SI{5}{\percent} of communication.}
	\label{fig:5percent_pend_top}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/stabilize/eval_model_param-5_commpen5-0_seed999_exemplary_rollout_improved.eps}
	\caption{Illustration of the performance of a learned communication and control policy that saves about \SI{90}{\percent} of communication.}
	\label{fig:90percent_pend_top}
	\end{subfigure}
\end{subfigure}
\caption{Exemplary rollouts of learned policies that save different amounts of communication. The agents are trained using the proposed algorithm.}
\label{fig:comm_savings_pend_top}
\end{figure}

\newpage

Since this task is linear, we can also compare our results to other well-known \gls{etc} algorithms. We linearize the pendulum around the upper equilibrium point and compare our approach to
\begin{itemize}
\item \textbf{LQR}: \\ $u[k] = K x[k] \Rightarrow \delta[k]=1 \text{ } \forall k \text{ ,}$
\item \textbf{LQR random skip}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \nu>\xi  \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $  
\item \textbf{state triggering 2 norm}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{x[k]}_2>\xi    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\item \textbf{output based triggering} \cite{6069816}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{K\hat{x}[k]-Kx[k]}_2>\xi \norm{Kx[k]}_2    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\item \textbf{state diff triggering} \cite{tabuada2007event}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{\hat{x}[k]-x[k]}_2>\xi \norm{x[k]}_2    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\end{itemize}
where $\hat{x}[k]$ represents the state at the last triggering instance and $\xi$ a threshold variable. I.e., by adjusting this threshold value, the triggering condition is altered, and therefore, the communication savings $\Gamma$ change. The random variable $\nu$, used in LQR random skip, is uniformly sampled from the interval $[0,1]$.

The gain matrix K is always chosen from the same LQR design with weigh matrixes $Q=\text{diag}([1.0,0.1])$ and $R=\begin{bmatrix} 0.1 \end{bmatrix}.$ This design choice again coincides with the parameters given by the standard OpenAI Gym implementation. Only the penalization on the control input has been increased from $0.001$ to $0.1$, to put more emphasis on a smooth control signal and to avoid to saturate the available input. The choice also ensures that the controller optimizes the same objective as the \gls{rl} agents \eqref{eq:ctrl_cost}.

\figref{fig:pareto_pend_top} shows the performance of the introduced event-triggering laws, together with the performance from our data-based \gls{rl} algorithm. As can be seen, for the classical approaches, only communication savings up to about \SI{80}{\percent} are possible, whereas our algorithm can come up with policies that can save up to \SI{90}{\percent}. However, for intermediate communication savings, the classical methods usually outperform our learning-based approach. This might be due to the fact that at these intermediate saving rates, there exist many local optima, and thus, our learning-based approach is prone to finding those suboptimal solutions. Nevertheless, the rewards of the classical approaches and our algorithm are in the same order of magnitude. In contrast, the learning approach introduced in \cite{BaumannRL} was also able to achieve communication savings of \SI{90}{\percent}, but was outperformed by orders of magnitude on intermediate communication savings.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{img/POC/stabilize/pareto.eps}
\caption{Illustration of the magnitude of $R_\text{ctrl}=-J_\text{ctrl}$ vs. the communication savings $\Gamma$ for various \gls{etc} strategies. For the learning agents, trained through the proposed algorithm, the best-trained policies have been selected. The mean and standard deviation are obtained by performing 10 rollouts with each of the policies.}
\label{fig:pareto_pend_top}
\end{figure}

The code for learning \gls{etc} from scratch and evaluating the models can be found at the git-amd server \footnote{\url{https://git-amd.tuebingen.mpg.de/nfunk/ppoc_off_tryout}}.

\newpage

\section{Stability Analysis and Retraining}

In the following section, we demonstrate how to show stability for \gls{nn} policies in the pendulum environment. The goal is to stabilize the pendulum in an upright position. Thus, we can obtain a linear system by linearizing the equations around the upper equilibrium point $\theta=\SI{0}{\degree}$ and $\dot{\theta}=\SI{0}{\degree / \second}$. The conversion from continuous to discrete-time is done using the matrix exponential method. 

For all of the following experiments, in line with Definition \ref{def:stability_def}, we define the safe state space ($\mathcal{O}$) to capture ranges of $\theta \in [\SI{-2.5}{\degree},\SI{2.5}{\degree}]$ and $\dot{\theta} \in [\SI{-5}{\degree / \second},\SI{5}{\degree / \second}]$. 

Usually, the state of the pendulum environment that is fed into the \gls{nn} to obtain the control action, is given by $x[k]=\begin{pmatrix} \cos(\theta[k]) & \sin(\theta[k]) & \dot{\theta}[k] \end{pmatrix}^T$. However, since for the stability verification algorithm we need to express the output of the \gls{nn} policy in terms of the variables of the system dynamics, \ie $\theta[k]$ and $\dot{\theta}[k]$, and can neither use the nonlinear sine nor the cosine function, we also linearize the state of the environment around the equilibrium which results in $x[k] \approx \begin{pmatrix} 1.0 & \theta[k] & \dot{\theta}[k] \end{pmatrix}^T$.

\subsection{Stability Analysis and Retraining - Periodic Control}

First, results for the stability analysis of \gls{nn} policies will be presented for the case when no resource constraints are active. Thus, we consider the setting of having one single \gls{nn} policy that simply outputs the action given the state.

For checking the stability of any \gls{nn} policy, one has to put them into the stability checking algorithm (\algref{alg:check_stab}). If the algorithm returns that there is not one single point violating the constraints, then this policy, in combination with the system dynamics, is considered to be stable. However, as \gls{nn} policies have many parameters and, therefore, also many degrees of freedom, it is obvious that this stability check is fulfilled very rarely. As shown in the previous chapter (\secref{sec:retrain_periodic}), the results from the stability analysis can be exploited to refine existing \gls{nn} control policies such that they fulfill the desired stability properties. This process is illustrated in \figref{fig:retrain_periodic_pendulum}, where a randomly initialized \gls{nn} policy is refined using \algref{alg:refine_pol}. After running the algorithm for 16 epochs, we arrive at a stable controller. Interestingly, although the stability retraining was only designed for an angular range of $\theta \in [\SI{-2.5}{\degree},\SI{2.5}{\degree}]$, the refined control policy also yields stable results when starting outside of this region.

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/only_comm/eval_model_param0_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum with a randomly initialized policy, for the case of periodic control, without any event-trigger. Each color represents a different rollout.}
	\label{fig:retrain_periodic_pendulum_l}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/only_comm/eval_model_param16_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum after retraining the policy with \algref{alg:refine_pol} for 16 epochs. The pendulum is now stabilized successfully. Each color represents a different rollout.}
	\label{fig:retrain_periodic_pendulum_r}
	\end{subfigure}
\end{subfigure}
\caption{Effect of the retraining procedure presented in \algref{alg:refine_pol}, for the case of  periodic control. After refining the randomly initialized policy for 16 iterations, a guaranteed stable controller is obtained, which successfully stabilizes the pendulum. While the initial controller (\figref{fig:retrain_periodic_pendulum_l}) is unstable, as the pendulum falls down, after applying the retraining, the controller is stable and the pendulum is kept upright (\figref{fig:retrain_periodic_pendulum_r}).}
\label{fig:retrain_periodic_pendulum}
\end{figure}

\subsection{Stability Analysis and Retraining - Event-triggered Control}

When also adding the communication decision into the stability check, the complexity of the check and retraining procedure doubles. The reason lies in the fact that we have to compute the next state for both of the cases, \ie for communicating and for not communicating (see \algref{alg:check_stability_ET_rigorous}). Then, the policy over options has to be evaluated to know whether the next state is inside the stable set or not. 

The results of running the retraining procedure are shown in \figref{fig:retrain_et_pendulum}. As one can see, after retaining for 4 iterations, a guaranteed stable controller is obtained, which successfully stabilizes the pendulum while still saving communication. Again, although we only trained for an angular region between \SI{-2.5}{\degree} and \SI{2.5}{\degree}, as shown in \figref{fig:retrain_et_pendulum_stable}, the policy also yields a stabilizing performance when starting outside of this interval. Over 10 randomly started runs, the policy saves around \SI{70}{\percent} of communication. An exemplary rollout of this very resource-efficient and guaranteed stable control policy can be seen in \figref{fig:retrain_et_pendulum_rollout}. To ensure that the refined policy still saves communication, it is important to include the constraint to skip communication whenever possible. Otherwise, the retraining procedure results in a policy that is always communicating.

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/full/eval_model_param0_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum with an \gls{et} policy, after 500 optimization epochs. Each color represents a different rollout.}
	\label{fig:retrain_et_pendulum_unstable}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/full/eval_model_param4_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum after retraining the policy with  \algref{alg:refine_pol} for 4 epochs. The pendulum is now stabilized successfully, while still saving communication. Each color represents a different rollout.}
	\label{fig:retrain_et_pendulum_stable}
	\end{subfigure}
\end{subfigure}
\caption{Effect of the retraining procedure presented in \algref{alg:refine_pol ET}, for the case of event-triggered control. While the initial policy is unstable (\figref{fig:retrain_et_pendulum_unstable}), after refining policy for 4 iterations, a guaranteed stable controller is obtained which successfully stabilizes the pendulum and still saves about \SI{70}{\percent} of communication (\figref{fig:retrain_et_pendulum_stable}).}
\label{fig:retrain_et_pendulum}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1.0\textwidth]{img/Marabou/full/eval_model_param4_exemplary_rollout.eps}
\caption{Illustration of an exemplary rollout of the same policy, as shown in \figref{fig:retrain_et_pendulum_stable}.}
\label{fig:retrain_et_pendulum_rollout}
\end{figure}

The code for the stability verification algorithm and retraining procedure can be accessed at \footnote{\url{https://git-amd.tuebingen.mpg.de/nfunk/ppoc_off_tryout}}.

\section{Learning Hierarchical, Periodic Control}

The application of our derived hierarchical \gls{rl} algorithm is not limited to the case of \gls{etc} only. One can also use this algorithm and equip both options with continuous control policies. In this short section, we provide results when both of the policies coincide with communication. The two options represent two different \glspl{nn} from which we can sample the actions. Further, we now consider the task of swingup and stabilization of the pendulum. We compare the results obtained by our algorithm with the original \gls{ppoc} implementation \cite{OptionCriticContPaper}, upon which we base our work. Choosing a hierarchical \gls{rl} framework is intuitive for this task as one could think of subdividing it into swingup and stabilization. 

\figref{fig:train_all_comparison} depicts the difference in the learning behavior between the \gls{ppoc} algorithm and our proposed approach. As can be seen in \figref{fig:training_all_comm_own}, the learning progress for our algorithm is way more stable compared to the \gls{ppoc} framework, see \figref{fig:training_all_comm_ppoc}. We think that the main reason for this gravely different behavior is that we also constrain the updates on the policy over options using PPO. One explanation, why this difference is so striking in the pendulum environment is that the reward changes gravely whenever the pendulum falls down. Therefore, using a rather smooth exploration strategy and limiting the updates for all of the policies involved, greatly stabilizes the learning process. A steady learning process is especially crucial in the \gls{et} setting, where the second option cannot compensate for anything but simply performs a \gls{zoh}. Thus, we think that our algorithm is better suited for \gls{etc}.

Nevertheless, the rollouts of the best performing policies, for both of the learning algorithms, result in comparable performance. Moreover, for both algorithms, only some of the policies exhibit the split behavior, \ie one option exclusively handling the swingup and the other one stabilizing the pendulum. 

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/all_comm/own_algo.eps}
	\caption{Training progress for swingup and stabilization of the pendulum using our own algorithm and two fully functional options.}
	\label{fig:training_all_comm_own}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/all_comm/ppoc.eps}
	\caption{Training progress for swingup and stabilization of the pendulum using the PPOC algorithm and two fully functional options.}
	\label{fig:training_all_comm_ppoc}
	\end{subfigure}
\end{subfigure}
\caption{Comparison of the learning progress for the two algorithms.}
\label{fig:train_all_comparison}
\end{figure}


==> chapters_old/0_Abstract.tex <==
% !TEX root = ../learning_et_ctrl.tex

% \begin{abstract}                          % Abstract of not more than 200 words.
% To support the flexibility and interconnectivity required by future engineering systems, increasingly more control loops will have to be closed using wireless or wired networks. It will therefore be key to come up with resource-efficient control algorithms that ensure sufficient performance without exceeding the available bandwidth. One approach to achieve this trade-off is the usage of event-triggered methods, consisting of a triggering law and a control policy. While the trigger determines when to communicate, the controller determines what to communicate. So far, state-of-the-art methods are usually either limited to linear and low-dimensional systems or optimize the two policies individually. Since future engineering systems are typically high-dimensional and nonlinear, and the separation principle does not hold in general, we present a data-driven, hierarchical reinforcement learning algorithm capable of learning event-triggered control strategies from scratch through jointly optimizing the policies. Without further modifications, our  method scales from simple, linear, to high-dimensional, nonlinear systems. Moreover, we showcase its potential on real hardware. Additionally, we describe a novel stability verification algorithm for neural network policies, applicable for both, periodic as well as event-triggered control and present results assuming linear system dynamics.
% \end{abstract}


%\begin{abstract}
%We present a framework for model-free learning of event-triggered communication and control policies from data.
%Event-triggered methods are essential to realize the potential of future networked control systems, where feedback loops are closed over wireless networks, and communication thus becomes a scarce resource. \st{I suggest saying more directly what ET methods are good for.  For example: With event-triggered methods, control updates happen spradically only when needed.  This allows for saving resources such as communication in NCS. Btw, NCS are not necessarily wireless}
%The learning approach jointly optimizes communication and control policy, which is required since the separation principle \st{unclear what separation principle is.  The abstract should be understandable also by non-experts} does not hold in general for event-triggered control, and can be applied to nonlinear and high-dimensional systems, as we demonstrate in challenging simulation examples.
%Further, we show in practical experiments on a robotic system that the method is also applicable to real-world systems and present an approach towards checking the stability of joint control and communication policies represented by deep neural networks.
%\st{Your sentences are rather long.  Try to use shorter sentences.  This is more common in Englisch.  Long sentences is German style. ;)}
%\st{Would be good to work out more clearly what the contribution of this article is.  Cf your contributions list below.  You might also want to give some technical details of your proposed method such as hierarchical RL}
%\end{abstract}

\begin{abstract}
We present a framework for model-free learning of event-triggered control strategies. 
% With event-triggered methods, control updates happen adaptively, only when needed.
Event-triggered methods aim to achieve high control performance while only closing the feedback loop when needed.
% This allows for saving resources such as communication and is essential to realize the potential of future networked control systems.
This enables resource savings, \eg network bandwidth if control commands are sent via communication networks, as in networked control systems.
Event-triggered controllers consist of a communication policy, determining when to communicate, and a control policy, deciding what to communicate.  
%is the case in networked control systems.
%To achieve both goals
It is essential to jointly optimize the two policies since individual optimization does not necessarily yield the overall optimal solution.
To address this need for joint optimization, we propose a novel algorithm based on hierarchical reinforcement learning.
%for learning event-triggered control.
% The main novelty is its ability to scale to nonlinear and high-dimensional systems, as we demonstrate in challenging simulation examples.
The resulting algorithm is shown to accomplish high-performance control in line with resource savings and scales seamlessly to nonlinear and high-dimensional systems. 
%without the need for any knowledge of the system dynamics.
% We also conduct practical experiments on a robotic system that show the method's applicability to real-world systems and present an approach towards checking the stability of the learned neural network policies. 
The method's applicability to real-world scenarios is demonstrated through experiments on a six degrees of freedom real-time controlled manipulator. Further, we propose an approach towards evaluating the stability of the learned neural network policies.
%The method's applicability to real-world scenarios is demonstrated through experiments on a robotic system. Further, we propose an approach towards evaluating the stability of the learned neural network policies.
%joint control and communication policies represented by deep neural networks.
%\st{Your sentences are rather long.  Try to use shorter sentences.  This is more common in Englisch.  Long sentences is German style. ;)}
%\st{Would be good to work out more clearly what the contribution of this article is.  Cf your contributions list below.  You might also want to give some technical details of your proposed method such as hierarchical RL}
\end{abstract}


==> chapters_old/1_IntroductionChapter.tex <==
% !TEX root = ../learning_et_ctrl.tex

\section{Introduction}
\label{chp:Introduction}

In modern control systems, control commands often need to be transmitted over (wired or wireless) communication networks~\cite{hespanha2007survey,lunze2014control}.
Examples of such networked control systems include swarms of drones, where communication is needed for drones to fly in formation; autonomous cars, where exchanging information between vehicles may increase traffic throughput and reduce fuel consumption; or smart homes, where distributed sensors, actuators, and computing units need to cooperate to regulate the indoor climate.
In all examples, multiple systems utilize the same network for communication.
If all systems transmit their information at high periodic rates, this can easily overload the network and result in an increased probability of message loss and longer transmission delays~\cite{7349192}.
Further, in many applications, distributed sensors and computing units should be untethered and thus battery-driven. In these cases, limiting communication can significantly improve battery life.
\Gls{et} methods have been developed explicitly to serve this need of controlling systems at reduced communication rates, see for instance~\cite{heemels2012introduction,miskowicz2018event,grune2014event,lemmon2010event} for an overview.

\begin{figure}
\centering
%\includegraphics[width=1.0\collen]{img/title/title_final1.png}
\includegraphics[width=1.0\collen]{img/title/title_img_code.pdf}
\caption{Performing event-triggered control on the Apollo robot. The overlayed frames coincide with the time instants in which a new control command is computed and applied. The robot successfully avoids the obstacle with only a few recomputations of the control signal and thus saving \SI{90}{\percent} of communication.}
\label{fig:title_hw_apollo}
\end{figure}
%\st{Not sure if comm symbol is clear in the context of this image?} 
%\st{The image looks a little "massive". Arm is too dark? Robot not visible?}
%\nf{Perhaps to be replaced with symbolic graphic}

In \gls{etc}, closing the feedback loop and, thus, transmitting information, is triggered by the occurrence of certain events, \eg an error growing too large.
Practical investigations have shown that \gls{etc} can significantly reduce the amount of communication while still achieving high-performance control~\cite{trimpe2011experimental,araujo2013system,dolk2017event}.
In most \gls{et} approaches, the design of the control and communication strategy is based on a known mathematical model of the system~\cite{heemels2012introduction}.
Yet, for complex systems, an accurate description may not be readily available.
Further, the majority of results only consider linear and low-dimensional systems.
Available results for nonlinear systems mostly optimize the  communication and control policies separately or fix one of both~\cite{demirel2018deepcas,vamvoudakis2018model}.
This is problematic as in \gls{etc}, the separation principle does not hold in general~\cite{ramesh2011dual}. That is: even if both policies are individually optimal, their combination does not necessarily yield the overall optimal solution.
For optimal \gls{etc}, the control and communication policy need to be optimized \emph{jointly}.
In this article, we propose an algorithm based on model-free \gls{rl} that jointly learns the control and communication policies from data. By exploiting model-free algorithms, we mitigate the need for an accurate dynamics model, and since we do not make any assumptions on dimensionality or linearity, the resulting framework can equally be applied to linear and nonlinear, low- and high-dimensional systems.

A key hurdle of learning \gls{etc} with \gls{rl} is the hybrid action space of such controllers.
At each time step, the controller takes a discrete decision, whether or not to communicate. In case of communication, a continuous control input is transmitted.
Hierarchical \gls{rl}~\cite{PrecupPHD} naturally captures this hybrid decision structure.
It provides a top-level policy that decides which action to take (in our case, whether or not to communicate). Depending on this choice, the corresponding low-level policy is evaluated, which, for instance, yields the control input in case of communication. To the best of our knowledge, hierarchical \gls{rl} has not yet been used for learning \gls{etc}. 
However, to successfully learn \gls{et} controllers, it is not sufficient to apply the existing hierarchical algorithms. This is mainly because the \gls{etc} setting restricts exploration. Unlike in periodic control, in \gls{etc}, varying the control action for exploration is only possible on communication
instances. Thus, exploration directly conflicts with the goal of saving communication. We extend the hierarchical algorithms accordingly, which results in the first method that successfully derives \gls{etc} strategies through joint optimization in nonlinear and high-dimensional environments.

%To the best of our knowledge, we are the first to leverage hierarchical \gls{rl} algorithms for \gls{etc} and the proposed method is the first that successfully derives \gls{etc} strategies through joint optimization in nonlinear and high-dimensional environments.


One of the drawbacks of learning-based approaches, especially those based on \glspl{nn}, is that they often do not provide stability guarantees. However, such statements are crucial when deploying the controllers at scale in potentially safety-critical, real-world applications.
We approach this challenge by proposing a verification framework, capable of checking the stability of the learned policy and refining it if necessary. 
% The algorithms are based on combining output range analysis of the learned control policy together with model knowledge. 
The framework combines output range analysis of the learned control policy with model knowledge.
That way, we can utilize a popular \gls{nn} verification framework~\cite{katz2017reluplex} to provide stability guarantees based on control invariant sets for linear systems.


\fakepar{Contributions} %\st{Overall, try to go a bit deeper and be more specific about your contributions! The related work section should elaborate and go into more detail in the comparison to literature.  There, it can be very effective to work out what aspects of your work are "the first" or "novel"}
% The contributions of this work can be summarized as follows:
We make the following contributions:
\begin{itemize}
\item Leveraging and extending hierarchical \gls{rl} algorithms to obtain resource-aware, \gls{et} controllers; 
\item Presenting an algorithm, capable of end-to-end learning of the control and communication policy through joint optimization for high-dimensional nonlinear systems;
\item Demonstrating the algorithm's practical significance by applying learned \gls{etc} strategies on a real robotic system, as illustrated in \figref{fig:title_hw_apollo};%\st{Can this be more specific?  What is it that you demonstrate?  High-dimensional?  very low communication?   What is the cool aspect about the experiments? Btw, aren't your simulations also a contribution?  E.g. high-dim + nonlinear?} 
\item Presenting an algorithm to check the stability of linear \gls{et} systems controlled by \gls{nn} policies with \gls{relu} activations. We also provide a method for refining the \glspl{nn} in case of initial instability.
%\item Development of an algorithm for refining \gls{nn} \gls{etc} policies to fulfill stability properties.\db{would combine the last two points}
\end{itemize}

\fakepar{Outline}
We start with an overview of related work before we provide the problem formulation and necessary background.
Next, we introduce the developed algorithm and present results in challenging, high-dimensional simulation environments and on a real robotic system.
Lastly, we discuss the stability verification procedure and conclude with a discussion.
% The article is structured as follows. First, we give an overview of related work before we provide the problem definition and background for the applied concepts. Second, we introduce the theory and developed methods. Third, results in high-dimensional, nonlinear simulation environments and on hardware, \ie the Apollo robot, are presented. Fourth, we outline the algorithms for checking the stability and potentially refining the obtained control policies. Last, we summarize the results and provide an outlook.

















% HERE I KEPT THE OLD CONTENT -> MAYBE TO BE ELIMINATED!!!
\begin{comment}
\subsection{Problem Formulation}
\label{sec:Int_Problem}

\subsubsection{Event-triggered Control}

Throughout the thesis, we consider a setting, as depicted in \figref{fig:etc_schematic}, where an actuator is acting on a physical system that is monitored by sensors. Without loss of generality, we assume the system dynamics to be given by 
\begin{equation}
x[k+1]=f(x[k],u[k],v[k]) \text{ ,}
\end{equation} 
where $x \in \mathbb{R}^n$ denotes the state, $u \in \mathbb{R}^m$ the input, $v \in \mathbb{R}^n$ additional process noise, and $k \in \mathbb{N}$ the discrete-time index. The measurements $y \in \mathbb{R}^p$ are assumed to be given by $y[k]=g(x[k],w[k])$, with $w \in \mathbb{R}^p$ representing measurement noise. The learning agent is directly connected to the sensors and continuously receives their measurements. Based on this information, the agent decides whether to communicate ($\delta[k]=1$) or not ($\delta[k]=0$) with the actuator - \ie whether to exploit the limited resources or to skip the current communication slot. Throughout the whole thesis, if not stated differently, we assume perfect communication conditions, \ie no delays in case of communication and no package losses. 

\begin{figure}
\centering
\includegraphics[width=0.75\collen]{img/Problem_Formulation/modified_schematic.png}
\caption{Schematic of the setting that is addressed in this thesis. Essentially, an actuator is acting on a physical system. The sensory information about the state of the system is delivered to a learning agent. The agent then has the choice to either communicate a control command to the actuator or to skip the current communication slot to save resources.}
\label{fig:etc_schematic}
\end{figure}

When the slot is skipped, and there is no communication between the agent and the actuator, a \gls{zoh} is performed at the actuator. This means that the control action is held constant, \ie the action communicated last is applied again. Mathematically, this can be written as
\begin{equation} \label{eq:zoh_gen}
\resizebox{.9\collen}{!}{$
u_{\text{ac}}[k] = \begin{cases} u_{\text{ag}}[k], & \text{if } \delta[k] = 1  \text{ , \ie communication} \\
u_{\text{ac}}[k-1], & \text{if } \delta[k] = 0 \text{ , \ie skipping communication} \text{ ,}
\end{cases}$}
\end{equation}
where $u_\text{ac}$ denotes the control action applied at the actuator and $u_\text{ag}$ represents the action calculated by the agent.

The communication savings $\Gamma$ can be expressed as the percentage of the available communication slots that have not been used, \ie $\Gamma = 1 - \frac{\sum_{k=1}^N \delta[k]}{N}$ for a trajectory of length $N$.

The goal of the thesis is to derive a learning algorithm that results in an optimal performance of the agent, as this is the fundamental unit in this setup. The agent has to come up with both a control and communication strategy that ensure that the physical system behaves in the desired way while the resource constraints (\ie not exploiting the limited communication bandwidth too extensively) are taken into account. Both objectives are combined in the following cost function
\begin{equation}
J = \sum_{k=0}^N \gamma^k (J_{\text{ctrl}}[k] + J_{\text{comm}}[k]) = \sum_{k=0}^N \gamma^k (J_{\text{ctrl}}[k] + \lambda \delta[k]) \text{ ,}
\label{eq:cost_fct}
\end{equation}

where $\lambda$ corresponds to the weight on penalizing communication, $\gamma$ to the discount factor, and $J_{\text{ctrl}}[k]$ to the control cost.

It is the goal of the learning algorithm to come up with a control and communication policy that minimizes the cost function \eqref{eq:cost_fct}.


\subsubsection{Stability Analysis of Neural Network Policies}

Most state-of-the-art, data-driven \gls{rl} algorithms for control are designed to optimize policies with many parameters. The approaches have shown impressive results in simulation studies. One of their main advantages is their generalization capability. The same algorithms can be deployed to simple, but also to high-dimensional nonlinear environments. However, the vast number of parameters makes it almost impossible to provide theoretical guarantees for the resulting control policies. In this thesis, we address this bottleneck and develop a stability check and retraining procedure for the resulting \gls{nn} control policies.

We define stability as finding a positive invariant set in the state space. I.e., once inside this set, when applying the \gls{nn} policy, the next state is guaranteed to also lie within this set. 
\\
\begin{defi}[Stability]{$\text{ }$\\}
The system $f$ is considered stable under the \gls{nn} control policy $u_\text{NN}[k]=h_\text{NN}(x[k])$ if there exists a region $\mathcal{O}$, such that \\
$x[k] \in \mathcal{O} \Rightarrow x[k+1]=f(x[k],h_\text{NN}(x[k])) \in  \mathcal{O} \text{ } \forall x[k] \in\mathcal{O}$.
\label{def:stability_def}
\end{defi}

\subsection{Thesis Outline}
\label{sec:Int_Outline}

\end{comment}

==> chapters_old/2_RelatedWorkChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section{Related Work}
\label{chp:RelatedWork}

%This paper presents an algorithm for model-free joint optimization of the communication and control policy for \gls{etc}. In this section, we relate the contributions to the literature.

\fakepar{\gls{etc} overview} For a general introduction and overview of \gls{etc}, we refer the reader to~\cite{lunze2014control,heemels2012introduction,miskowicz2018event,lemmon2010event}. 
While~\cite{heemels2012introduction} focuses on linear systems, the other references also discuss approaches for event-triggered control of nonlinear systems.
All methods, regardless of whether they are designed for linear or nonlinear systems, rely on an accurate model of the system's dynamics.
In practical applications, especially when considering complex nonlinear systems, such a model may not be available.
We address the more general and more challenging problem of learning event-triggered control and communication policies without assuming any knowledge of the system dynamics. 
% Steve comment: RL more general but simpler to implement than nonlinear control therefore maybe do away last sentence?
%\db{maybe add sth about dimensionality}

%\fakepar{Learning \gls{etc}}
%\db{If you want to use the fakepars, you should have one per abstract. So here you would need to group the different approaches for learning \gls{etc}, \eg with fixed threshold vs. without imposing a structure} 

%While many \gls{et} algorithms exist and have shown good performance \cite{heemels2012introduction,grune2014event}, guaranteeing optimality is non-trivial as the separation principle does not hold in general \cite{ramesh2011dual}.
%\db{If we want to have a paragraph on general event-triggered control, then this needs to be longer.
%We would need to cite some survey papers and state that the methods therein only work for linear systems.
%Then we would need to discuss some works on nonlinear event-triggered control and for each of them discuss, what they lack (only low-dimensional, no joint optimization, \ldots)

%Generally, it would be nice to structure this section a bit using for instance fakepars.
%You could have \fakepar{learning \gls{et} control policies}, \fakepar{joint learning}, \fakepar{Deep \gls{rl} for learning control}, \fakepar{stability analysis} (titles would need to be adjusted, but just to give you an idea)}

%Recently, there have been several attempts towards jointly optimizing control and communication strategy for \gls{etc}.
% In view of the advance of \gls{ncs}, \gls{et} methods recently arouse a lot of interest \cite{heemels2012introduction,grune2014event}. They provide means to resolve the contradiction between resource-efficiency and performance and have been used for all sorts of purposes from state-estimation \cite{trimpe2011experimental} to planning \cite{1242252} and control \cite{trimpe2015event}.
% \db{Here we should probably have some more references, also from other groups.
% I can do that later} 
% While many \gls{et} algorithms exist and have shown good performance, guaranteeing optimality is non-trivial as the separation principle does not hold in general \cite{ramesh2011dual}. The design of an optimal controller combined with an independently designed optimal communication scheme does not necessarily yield the optimal solution. Thus, it is crucial to apply a joint optimization procedure for communication and control strategy.
% \db{This paragraph I would skip here and already have this in the introduction (see my comment there)}
% Lately, there have been several attempts to solve this joint optimization problem in a model-free way. 
\fakepar{Learning \gls{etc} -- imposing structure} Recently, there have been several other works that learn \gls{et} communication and control policies in a model-free way. In \cite{demirel2018deepcas}, the authors propose to use \gls{rl} to learn a scheduling strategy for controlling a multi-agent system. 
The approach focuses on arbitrating the constrained communication bandwidth among the agents, while the agents' control strategy is fixed beforehand and not subject to active optimization. 
Vamvoudakis et al. \cite{vamvoudakis2018model} exploit concepts from Q-learning, and propose a model-free algorithm that comes up with an \gls{etc} strategy for linear systems in continuous time. 
In their approach, the general triggering condition is predefined. Therefore, the optimization algorithm only operates on the triggering threshold of the communication strategy (\ie when to trigger). 
The authors of \cite{zhong2014event} and \cite{yang2017event} also use the same predefined triggering condition, but derive \gls{etc} strategies for nonlinear systems. 
While \cite{zhong2014event} uses an adaptive dynamic programming approach, \cite{yang2017event} relies on an identifier-critic architecture, actively identifying the unknown system dynamics. 
The authors of \cite{sahoo2015neural} use \glspl{nn} to parametrize the control policy, while the triggering condition depends on the state and the weights of the controller. 
Further, the \gls{nn} is updated in an aperiodic fashion, \ie only on triggering instances. 
The method proposed herein is more general. We jointly learn the control and communication strategy from scratch without imposing any additional structure, \eg concerning the triggering condition. This is especially crucial as the separation principle does not hold in general for \gls{etc} \cite{ramesh2011dual}. Moreover, we showcase the performance of our algorithm in substantially more complex and higher-dimensional simulation environments than those presented in the above references, as well as on a real 6 \gls{dof} real-time controlled manipulator.
% Nevertheless, we are still capable of presenting a stability analysis for the resulting policies\db{with this statement I would be careful, since we cannot analyze the stability of the nonlinear systems}. Moreover, compared with \cite{vamvoudakis2018model}, the herein presented learning algorithm can be applied straightforwardly to nonlinear systems.

\fakepar{Learning \gls{etc} -- without imposing structure} There are only few other approaches~\cite{BaumannRL,hashimoto2019learning} that learn ETC without a-priori restrictions on the triggering condition. Baumann et al.~\cite{BaumannRL} discuss both a joint optimization of control and communication and a separate optimization procedure.
However, only the separate optimization can be applied to high-dimensional tasks.
The authors of~\cite{hashimoto2019learning} propose to use Gaussian processes to learn a model of an unknown system, which is then exploited to derive an optimal, self-triggered control strategy through approximated value iteration.
Due to the computational complexity, this approach is limited to low-dimensional systems, and a maximum inter-communication time needs to be fixed a priori.
Thus, neither of those approaches can jointly optimize the control and communication policy in high-dimensional settings, as we do herein.
Further, neither work provides any stability guarantees or results on real hardware.

% Both\db{Other approaches that learn ETC without \ldots can be found in}, \cite{BaumannRL} and \cite{hashimoto2019learning} present data-driven approaches for learning \gls{et} control, without pre-specifying any triggering condition. However, the increased flexibility comes at the cost of not being capable of providing stability guarantees and theoretical analysis contrarily to our and the previously presented approaches. Also, as opposed to this work, both of the algorithms cannot scale to high-dimensional environments.\db{In my CDC paper we also present a high-dimensional example. I know what you mean, but probably need to formulate this a bit more carefully here.}

% In \cite{hashimoto2019learning}, the authors propose to use Gaussian processes to learn a model of an unknown system which is then exploited to derive an optimal self-triggered control strategy using approximate value iteration. In their approach, the maximum inter-communication time has to be fixed a priori, and due to the computational complexity, this approach is currently limited to low-dimensional systems. Baumann et al. \cite{BaumannRL}\db{You're discussing my paper two times, can skip one of them} transfer the concept of end-end learning  \cite{levine2016end} to the \gls{etc} setting and present a deep \gls{rl} algorithm based on DDPG \cite{lillicrap2015continuous}, which is capable of jointly learning a control and communication strategy. So far, the joint optimization from scratch does not work for high-dimensional systems and no stability results are presented. \db{ok, that way it's fine, just delete my paper from the previous paragraph}

\fakepar{Deep \gls{rl} for learning control} Learning control policies from data for high-dimensional and nonlinear systems has been studied extensively in recent years~\cite{lillicrap2015continuous,duan2016benchmarking,levine2016end,peters2008reinforcement,kober2013reinforcement}.
However, all these works consider periodic communication and are, therefore, not applicable to the problem considered herein.
\gls{etc} is a challenging problem in that it leads to a hybrid action space.
%we have a discrete communication decision and a continuous control action.
Approaches that deal with such hybrid action spaces will be discussed next. %can be found in~\cite{BaumannRL,neunert2020continuous,SuttonTDLearning,PrecupPHD,OptionCriticPaper}\db{would leave this out and simply say will be discussed next. If you want to keep it, you should probably also include~\cite{masson2016reinforcement,hausknecht2016deep} in this list}.
In~\cite{masson2016reinforcement,hausknecht2016deep}, the authors propose to rephrase the problem using continuous variables following the concept of a parameterized action space Markov decision process.
This approach has been used to jointly learn communication and control policies in~\cite{BaumannRL}. Yet, it has only been shown to be successful in low-dimensional tasks.
More recently,~\cite{neunert2020continuous} introduced a hybrid \gls{rl} algorithm that can optimize such problems without reformulation.
So far, this has not been applied to \gls{etc}.
Hierarchical \gls{rl} frameworks~\cite{PrecupPHD,SuttonTDLearning,OptionCriticPaper} represent a third approach to address the hybrid problem setting. Originally, the hierarchical structure stems from the concept of temporal abstraction. However, it also naturally captures the structure of \gls{etc}. 
The discrete high-level decision on which sub-policy to execute next coincides with the communication decision in \gls{etc}, while the sub-policy yields the continuous control command.      
We are not aware of any other work that extends hierarchical \gls{rl} algorithms to make them applicable for \gls{etc}, as we do herein.

% Previous Version:
%A third approach that addresses hybrid problem settings is given by hierarchical \gls{rl} frameworks~\cite{SuttonTDLearning,PrecupPHD,OptionCriticPaper}. Initially, the hierarchical structure 
%The hierarchical approach naturally captures the \gls{etc} problem.
%We have a high-level decision on whether to communicate and, based on this decision, need to apply a control command.
%Thus, in this work, we extend hierarchical \gls{rl} algorithms to make them applicable for \gls{etc}.

\fakepar{Stability analysis} Due to the nonlinear activation functions and many parameters involved, it is usually difficult to provide stability guarantees for learned policies parametrized by \glspl{nn}. Thus, this problem is typically not addressed. Two recent exceptions related to the approach herein are~\cite{bonassi2019lstm} and~\cite{karg2020stability}. In~\cite{bonassi2019lstm}, the authors guarantee input to state stability of long short term memory \glspl{nn}. This can effectively be exploited when using \glspl{nn} for modeling or system identification. Its use for controller design has not yet been demonstrated. 
Karg et al. \cite{karg2020stability} examine the stability of \gls{nn} controllers via output range analysis. This way, they can model the closed-loop behavior of the controlled system and define requirements for asymptotic stability. To achieve this property, they propose to refine the final layer of the \gls{nn}, based on a predefined linear quadratic regulator policy. Our approach is more general in that it refines the entire network instead of only the final layer and is not restricted to a particular type of controllers.
Further, compared to both approaches, we provide results for larger networks and present an approach for checking the stability of \gls{etc} policies, which is generally more challenging due to the sporadic updates, triggered by the communication policy.

%While both approaches only consider the periodic control problem, we present a novel stability verification algorithm and retraining procedure for the case of \gls{etc}. Further, we provide results for larger networks. Compared to \cite{karg2020stability},  

%Compared to \cite{karg2020stability}, our approach is also output-based but end-to-end in the way that it refines the entire network and does not rely on the additional design of a controller.

%To the best of our knowledge, we are the first to present a stability verification and retraining procedure for \gls{nn} \gls{etc} policies that have been obtained through \gls{rl}.  



% Due to the discrete communication decision and the continuous control action to be applied, \gls{etc} represents a hybrid control problem, which is difficult to solve for most standard \gls{rl} algorithms. One way to get rid of the hybridity is to rephrase the problem using continuous variables only by following the concept of a parameterized action space Markov decision process (PAMDP) \cite{masson2016reinforcement}. More recently, \cite{neunert2020continuous} introduced a hybrid \gls{rl} algorithm that can optimize such problems without reformulation. A third approach is to use a hierarchical \gls{rl} framework \cite{OptionCriticPaper}, which naturally captures the \gls{etc} problem formulation. Our approach makes use of the hierarchical approach as its special structure, having separate policies for the discrete and continuous control decision, allows to save computational resources during runtime. Further, to the best of our knowledge, these existing approaches, if used for control, are without stability analysis, and hierarchical \gls{rl} methods have not been considered for \gls{etc} yet.  
% \db{Restructure: After introducing the three possibilities, say that none of those have been used for ETC, then say that we use hierarchical RL as the basis for our algorithm}



==> chapters_old/3_0_ProblemDefinitionChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section{Problem Formulation}
\label{sec:ProblemDefinition}

%In this section, we define the problem setting. We first discuss the considered class of systems and performance objectives. Then, we introduce the main idea of the learning algorithm.

%\nf{perhaps also reiterate this figure}
%\st{The drawing is not very rich in terms of information that is conveyed.  Also, I'm wondering if it is a good representation.  It looks like the learning agent decides online whethre to communicate or not.  But that's not the case.  So, how about having a control/communication agent, and then a learning/RL "loop" around this?  This would also make the image richer and allow you to include details like what data is used in the RL, what decisions are made, etc. I think it makes sense to spend some thoughts on developing a nice drawing that is representative for this work. }

% We consider a setting, as depicted in \figref{fig:etc_schematic}. 
% where an actuator is acting on a physical system that is monitored by sensors. 
% The actuator receives the control commands from the learning agent via a communication network.

\fakepar{System} We consider a dynamic system whose state is monitored by sensors, and that is connected to a learning agent (\cf\figref{fig:etc_schematic}). While the sensor measurements are directly available to the learning agent, control commands need to be transmitted over a communication network to the actuators. If not stated differently, we assume the dynamics of the system to be unknown and of the form 
\begin{equation}
x[k+1]=f(x[k],u[k],v[k]) \text{ ,}
\end{equation}
where $x[k] \in \mathbb{R}^n$ denotes the state, $u[k] \in \mathbb{R}^m$ the input, $v[k] \in \mathbb{R}^n$ process noise, and $k \in \mathbb{N}$ the discrete-time index. The measurements $y[k] \in \mathbb{R}^p$ are assumed to be given by 
\begin{equation}
y[k]=g(x[k],w[k]) \text{ ,}
\end{equation}
with $w[k] \in \mathbb{R}^p$ representing measurement noise. %While we consider perfect communication and no delays in simulation environments, we will also test our method under real experimental conditions with delays and potential packet losses.

\begin{figure}
\centering
%\includegraphics[width=1.0\collen]{img/Problem_Formulation/Overview1.png}
\includegraphics[width=1.0\collen]{img/Problem_Formulation/Overview.pdf}
\caption{Schematic of the learning \gls{etc} setting addressed in this article. An actuator is acting on a physical system. The sensory information about the state of the system is delivered to the learning agent. The agent then has the choice to either communicate a control command to the actuator ($\delta=1$) or to skip the current communication slot to save resources ($\delta=0$). The communication decision is retrieved from \gls{nn} $\mu$. In case of communication, the control action is computed via \gls{nn} $\pi$. During training time, the weights of the \glspl{nn} are refined via backpropagation.}
\label{fig:etc_schematic}
\end{figure}

\fakepar{Event-triggered control} Unlike in periodic control, in \gls{etc} the feedback loop is closed adaptively. Based on the measurements, the agent decides whether ($\delta[k]=1$) or not ($\delta[k]=0$) to communicate with the actuator - \ie whether to exploit the limited resources or to skip the current communication slot. 
% When the slot is skipped, a \gls{zoh} is performed at the actuator, otherwise, the agent provides the control action to be applied. 
As is typically done in \gls{etc}~\cite{heemels2012introduction}, we assume \gls{zoh} at the actuator in between communication events.
Mathematically, this can be expressed as
\begin{equation} \label{eq:zoh_gen}
u_{\text{ac}}[k] = \begin{cases} u_{\text{ag}}[k], & \text{if } \delta[k] = 1 \\
u_{\text{ac}}[k-1], & \text{if } \delta[k] = 0 \text{ ,}
\end{cases}
\end{equation}
where $u_\text{ac}$ denotes the control action applied at the actuator and $u_\text{ag}$ represents the action calculated by the agent (cf. \figref{fig:etc_schematic}). 

\fakepar{Performance objective} The proposed learning algorithm  should result in both a control and communication strategy that ensure that the physical system behaves in the desired way (\eg reaching a desired setpoint) while the resource constraints are taken into account. Both objectives are combined in the following reward function
\begin{equation}
\begin{split}
R &= \sum_{k=0}^N \gamma^k (R_{\text{ctrl}}[k] + R_{\text{comm}}[k])\\ 
&= \sum_{k=0}^N \gamma^k (R_{\text{ctrl}}[k] - \lambda \delta[k]) \text{ ,}
\label{eq:cost_fct}
\end{split}
\end{equation}
where $\lambda$ is the weight on penalizing communication, $\gamma$ the discount factor, and $R_{\text{ctrl}}[k]$ the control reward. If the discount factor $\gamma$ is less than 1, it limits the horizon up to which future rewards are reflected in the value of the function. We express the communication savings $\Gamma$ as the percentage of the available communication slots that have not been used, \ie 
\begin{equation}
\Gamma = 1 - (\sum_{k=1}^N \delta[k])/N
\end{equation}
for a trajectory of length $N$. That is, $\Gamma = \SI{100}{\percent}$ means all communication slots have been used, and $\Gamma = \SI{0}{\percent}$ corresponds to no communication.

\fakepar{Problem statement} 
% In this paper, we seek to derive a learning algorithm that results in an \gls{et} control strategy that maximizes~\eqref{eq:cost_fct}.
The goal of this paper is to devise a learning algorithm that maximizes~\eqref{eq:cost_fct}.
To address the drawbacks of existing methods, the algorithm shall meet the following requirements: \emph{(i)} it should be model-free to avoid the need for an accurate dynamics model; \emph{(ii)} it should jointly optimize the control and communication policy since the separation principle does not hold in general for \gls{etc}; \emph{(iii)} it should be applicable to linear and nonlinear, \emph{(iv)} low- and high-dimensional systems.

\fakepar{Towards stability} In addition to learning \gls{etc}, which is the focus of this work, we are also concerned with providing stability guarantees for the policies. This is essential for the practicability of the method, especially considering its potential use in safety critical environments. However, this is particularly difficult when dealing with learned, highly parametric, and nonlinear \gls{nn} control strategies in the \gls{etc} setting. We approach this challenge by defining system stability through control invariant sets, assuming known, linear dynamics, and using \glspl{nn} with \gls{relu} activations. This allows us to devise a second algorithm capable of verifying and refining the \gls{nn} policies to guarantee system stability.  



%\fakepar{Towards stability} Besides deriving the algorithm, we also want to address the challenge of providing stability guarantees for the learned policies. This is essential for the practicability of the method, especially considering its use in safety critical environments. However, this is particularly difficult when dealing with learned, highly parametric and nonlinear \gls{nn} control strategies in the \gls{etc} setting. In this work, we want to approach this challenge by defining stability through control invariant sets and exploiting model knowledge. %we can present a first stability verification algorithm for the policies in \secref{sec:stability_statment}.\db{This is not part of the problem statement, but of the contributions. If you want to have it as part of the problem statement, need to leave out the last sentence and state this as a further requirement}    

%In the following two sections, we focus on the learning algorithm and propose an approach based on hierarchical \gls{rl}, which fulfills the desired properties, successfully derives \gls{etc} strategies from scratch through joint optimization and scales from simple to very complex environments.
%\db{You already provided an outline at the end of the intro, so this paragraph is probably not necessary}

==> chapters_old/3_BackgroundChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

%\section{Background}
%\label{chp:Background}

%We now introduce the necessary concepts from \gls{rl} upon which we %base our work.   

\section{Background: Hierarchical Reinforcement Learning}
\label{sec:hrl}

%\gls{etc} represents a hybrid control problem, which is difficult to solve for most standard \gls{rl} algorithms. In contrast, the structure of hierarchical \gls{rl} can be exploited to split the discrete and continuous variables, therefore, significantly simplifying the learning process. Thus, in the following, we introduce the options framework \cite{PrecupPHD,SuttonTDLearning,OptionCriticPaper}, a hierarchical \gls{rl} framework established by Precup et al.. 

\gls{etc} represents a hybrid control problem, which is difficult to solve for most standard \gls{rl} algorithms.
In the following, we introduce the options framework established by Precup \etal~\cite{PrecupPHD,OptionCriticPaper}. 
This hierarchical \gls{rl} framework is particularly suitable for learning control policies in hybrid action spaces as it naturally splits the discrete and continuous variables.
%Instead of having one single policy that is queried at every timestep, a set of policies is used on different levels. A simple setting could be, having one high-level policy that decides which of the two low-level policies calculates the control action. This structure allows to split the discrete and continuous variables and therefore simplifies the learning process. Using a hierarchical approach also allows to save computational resources as not all policies have to be evaluated at each timestep. Thus, in the following, we introduce the options framework \cite{PrecupPHD,SuttonTDLearning,OptionCriticPaper}, a hierarchical \gls{rl} framework established by Precup et al..\db{I would shorten this paragraph and say that how to apply it to \gls{etc} will be discussed in the next section.}

%Due to the discrete communication decision and the continuous control action to be applied, \gls{etc} represents a hybrid control problem, which is difficult to solve for most standard \gls{rl} algorithms. In contrast, the structure of hierarchical \gls{rl} algorithms captures the hybrid setting. Instead of having one single policy that is queried at every timestep, a set of policies is used on different levels. A simple setting could be, having one high-level policy that decides which of the two low-level policies calculates the control action. This structure allows to split the discrete and continuous variables and therefore simplifies the learning process. Using a hierarchical approach also allows to save computational resources as not all policies have to be evaluated at each timestep. Thus, in the following, we introduce the options framework \cite{PrecupPHD,SuttonTDLearning,OptionCriticPaper}, a hierarchical \gls{rl} framework established by Precup et al..\db{I would shorten this paragraph and say that how to apply it to \gls{etc} will be discussed in the next section.}

%The general motivation behind hierarchical \gls{rl} is the concept of temporal abstraction. Instead of having one single policy that is queried at every timestep, a set of policies is used on different levels. A simple setting could be, having one high-level policy that decides which of the two low-level policies calculates the control action. This enables to better capture processes that run on different time scales and to potentially save computational resources as not all policies have to be evaluated at each timestep. From a different perspective, the hierarchy can also be viewed as separating the action space, \ie the final control action to be applied is made up of decisions on various levels. As we are dealing with a hybrid action space, a discrete communication decision together with a continuous control action to be applied, this setting is naturally captured by hierarchical \gls{rl} algorithms. Thus, in the following, we introduce the options framework \cite{PrecupPHD,SuttonTDLearning,OptionCriticPaper}, a hierarchical \gls{rl} framework established by Precup et al..

To represent the hierarchy, the options framework requires one additional variable, called option $o$, besides the state $x$ and the control action $u$. The framework is parametrized by three policies: the policy over options $\mu(o_i|x)$, the intra option policy $\pi_{o_i}(u|x)$, and the termination function $\beta_{o_i}(x)$. The principle in few words: the policy over options decides which option is to be executed. Depending on this choice, the action is sampled from the corresponding intra option policy until the termination function indicates to stop the execution of the current option, which triggers a restart of the procedure. Mathematically, the policy over options $\mu(o_i|x)$ determines the probability of choosing option $o_i$, the intra option policy $\pi_{o_i}(u|x)$ determines the distribution over actions $u$, and the termination function $\beta_{o_i}(x)$ determines the probability for terminating the execution of option $o_i$. As shown in \cite{SuttonTDLearning}, this can be rephrased as having a flat action space without the hierarchy,
\begin{equation} \label{eq:conv_flat}
\pi(u|x,o)=(1-\beta_o(x))\pi_o(u|x) + \beta_o(x) \sum_{\tilde{o}}^{} \mu(\tilde{o}|x) \pi_{\tilde{o}}(u|x) \text{ .}
\end{equation} 

To optimize the agent's behavior, it is essential to estimate the expected reward of its actions using the Q-function. This estimate directly indicates which actions are more rewarding. In standard \gls{rl}, the Q-function assigns a value to a state-action pair $(x,u)$. In the hierarchical setting, we define it as assigning a value to a state-option pair $(x,o)$,
\begin{equation}
Q(x_i,o_i)= \sum_{\tilde{u}}^{} \pi_{o_i}(\tilde{u}|x_i) \tilde{Q}(x_i,o_i,\tilde{u}) \text{ ,}
\label{eq:Q-fct-hierarchicalrl}
\end{equation} 
where $\tilde{Q}$ can be computed via $\tilde{Q}(x_i,o_i,u)=r(x_i,o_i,u)+\gamma Q(x_{i+1},o_{i+1})$ and $r$ defines the single step reward. In conclusion, the Q-function describes the future reward to be expected when starting from state $x_i$ and option $o_i$.

% The goal of the algorithm is to maximize the expected reward. 
The options framework aims at maximizing the expected reward, which for a given state $x_i$ and option $o_i$ reads
% Given a state $x_i$ and the current option $o_i$, the reward accounts to 
\begin{equation}
\label{eq:reward_def}
\begin{split}
R(x_i,o_i) &=[1-\beta_{o_i}(x_i)]Q(x_i,o_i) \\
&+\beta_{o_i}(x_i) \sum_{\tilde{o}}^{} \mu(\tilde{o}|x_i) Q(x_i,\tilde{o}) \text{ .}
\end{split}
\end{equation}
Assuming the termination function $\beta$ is parametrized by parameters $\theta_\beta$, the policy over options $\mu$ by $\theta_\mu$, and the intra option policy $\pi$ by $\theta_\pi$, the gradient of the reward \eqref{eq:reward_def} with respect to the policies is given by
\begin{equation}
\begin{split}
&\frac{\partial R(x_i,o_i,\theta_\beta,\theta_\mu)}{\partial \theta_\mu}\\ 
&= \beta_{o_i}(x_i,\theta_\beta) \mathbb{E}[\frac{\partial}{\partial \theta_\mu} \log(\mu(o_i,\theta_\mu|x_i))Q(x_i,o_i)]
\end{split}
\label{eq:vanilla_grad_pol_op}
\end{equation}
%\begin{comment}
%&= \beta_{o_i}(x_i,\theta_\beta) \sum_{\tilde{o}}^{} \frac{\partial \mu(\tilde{o},\theta_\mu|x_i)}{\partial \theta_\mu} Q(x_i,\tilde{o}) \\ 
%\end{comment}
and
\begin{equation}
\begin{split}
&\frac{\partial R(x_i,o_i,\theta_\beta,\theta_\mu)}{\partial \theta_\beta} =\\
& \frac{\partial \beta_{o_i}(x_i,\theta_\beta)}{\partial \theta_\beta} (\sum_{\tilde{o}}^{} \mu(\tilde{o},\theta_\mu|x_i) Q(x_i,\tilde{o}) - Q(x_i,o_i)) \text{ .}
\end{split}
\label{eq:vanilla_grad_term}
\end{equation}

For each intra option policy, we seek to maximize
\begin{equation}
Q(x_i,o_i)=\sum_{u}^{} \pi_{o_i}(u,\theta_\pi|x_i)\tilde{Q}(x_i,o_i,u) \text{ .}
\end{equation}
Taking the gradient results in 
\begin{equation}
\frac{\partial Q(x_i,o_i,\theta_\pi)}{\partial \theta_\pi} = \mathbb{E}[\frac{\partial}{\partial \theta_\pi} \log(\pi_{o_i}(u,\theta_\pi|x_i))\tilde{Q}(x_i,o_i,u)] \text{ .}
\end{equation}

%PPO has proven to stabilize the learning process for continuous action tasks by limiting the covariate shift. and is closely related to trust region methods such as \gls{trpo} \cite{TRPOPaper}. Compared to TRPO, PPO is easier to implement and exhibits similar performance, however, at the cost of losing strict performance guarantees\db{I would skip this discussion about TRPO}.

For continuous action spaces, \cite{OptionCriticContPaper} proposes to use \gls{ppo} \cite{PPOSchulman} for updating the intra option policy. PPO stabilizes the learning process for continuous action tasks by limiting the covariate shift through including a clipping function into the optimization objective $L$. Let $\theta$ denote the parameters to be optimized, and $\pi'$ denote the new policy to be found ($\pi'=\pi(\theta)$), whereas $\pi$ denotes the policy under the old parameters ($\pi=\pi(\theta_\text{old})$) which were used for sampling the state action transitions. The goal of the \gls{ppo} algorithm is to optimize 
\begin{equation}
\begin{split}
L(\pi') &= R(\pi')-R(\pi) \\
&=r(x_i,o_i,u^{\pi'})+\gamma Q^{\pi}(x_{i+1},o_{i+1}) - Q^{\pi}(x_i,o_i) \\
&=A^{\pi}(x_i,o_i,u^{\pi'}) \approx \frac{\pi_o'(u|x)}{\pi_o(u|x)} A^{\pi}(x_i,o_i,u^{\pi}) \text{ .}
\end{split}
\end{equation}
Following the derivations presented in \cite{OptionCriticContPaper}, we have
% the \gls{ppo} update for the intra option policy is given by 
\begin{equation}
\begin{split}
\frac{\partial L(\theta)}{\partial \theta} &= \mathbb{E} [\frac{\partial}{\partial \theta} \min[\frac{\pi_o'(u|x)}{\pi_o(u|x)} A^{\pi}(x,o,u^{\pi}) , \\ 
&\text{clip}(\frac{\pi_o'(u|x)}{\pi_o(u|x)},1-\epsilon,1+\epsilon) A^{\pi}(x,o,u^{\pi})]] 
\end{split}
\label{eq:ppo_pol_op}
\end{equation}
for the update of the intra option policy, with the advantage $A^{\pi}(x_i,o_i,u^{\pi})=r(x_i,o_i,u^{\pi})+\gamma Q^{\pi}(x_{i+1},o_{i+1})- Q^{\pi}(x_i,o_i)$, and the clipping function
% where $\epsilon$ determines the range where no clipping is applied, and the clipping function is defined as
\begin{equation}
\text{clip}(a,b,c) = \begin{cases} a, & \text{if } a \in [b,c] \\
b, & \text{if } a < b \\
c, & \text{if } a > c \text{ ,} 
\end{cases}
\end{equation}
assuming $c \geq b$, and $\epsilon$ the range in which no clipping is applied.

Combining \eqref{eq:vanilla_grad_pol_op}, \eqref{eq:vanilla_grad_term}, and \eqref{eq:ppo_pol_op} leads to the \gls{ppoc} framework for continuous action spaces, as presented in \cite{OptionCriticContPaper}. Further, \cite{OptionCriticContPaper} uses \gls{gae} \cite{schulman2015GAE} to calculate $A^{\pi}(x,o,u^{\pi})$. The GAE algorithm allows to tune the bias-variance tradeoff when estimating this advantage term. 
%\nf{In my opinion, maybe we can omit the clipping function? Interested readers can just refer to the PPO paer but it also does not consume too much space,...}
%\db{I think it's fine to leave it in}

==> chapters_old/4_TheoryAndMethodsChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section[Learning Event-triggered Control and Communication Policies]{Learning Event-triggered Control and \\ Communication Policies}
\label{sec:leveragingrl_etc}

We now establish the link between the previously introduced hierarchical \gls{rl} algorithm and the \gls{etc} problem formulation and present an algorithm capable of learning \gls{etc} strategies from data through joint optimization. In \secref{sec:mergin} we bridge the gap between ETC and hierarchical RL and show in which ways the problems they solve are related. In \secref{sec:leveragingrl_etc} we first explain why simply applying plain hierarchical \gls{rl} is not enough to solve \gls{etc} problems before we show how existing algorithms and concepts need to be extended to be applicable.% to \gls{etc}.

\subsection{Relating Hierarchical Reinforcement Learning to Event-triggered Control}
\label{sec:mergin}

The hierarchical \gls{rl} algorithm presented in the preceding section naturally allows us to represent problems with hybrid action spaces. The policy over options $\mu$ performs a discrete decision (which option to execute next), while the intra option policy $\pi_o$ returns a continuous action, if needed. Thus, in the context of \gls{etc}, the policy over options represents the triggering law, while the intra option policy yields the control action in case of communication.
We always assume that option 0 ($o_0$) corresponds to no communication and to performing the \gls{zoh}, while option 1 ($o_1$) corresponds to sampling a continuous action from a \gls{nn} policy, \ie $u_\text{ag}[k]=\pi_{o_1}(u|x)$ (\cf~\eqref{eq:zoh_gen}).
Thus, the \gls{et} policy saves not only communication, but also computational resources since the intra option policy does not need to be evaluated in case of no communication.
% Recalling \eqref{eq:zoh_gen}, for the case of having the two previously introduced options, this can be summarized as 
Using this definition of options,~\eqref{eq:zoh_gen} can be rewritten as
\begin{equation} \label{eq:zoh_gen_opt}
u_{\text{ac}}[k] = \begin{cases} u_{\text{ac}}[k-1], & \text{if } \delta[k] = 0 \text{, } o=o_0  \\
u_{\text{ag}}[k]=\pi_{o_1}(u|x), & \text{if } \delta[k] = 1 \text{, } o=o_1 
\text{ .}
\end{cases}
\end{equation}

%\nf{Sebastian proposed another title but IMO, the linking aspect fits very well here as the concepts are merged.}

\subsection{Hierarchical Reinforcement Learning for Event-triggered Control}
\label{sec:leveragingrl_etc}

%For the purpose of learning \gls{etc} from data, we propose the following modifications to the original \gls{ppoc} algorithm \cite{OptionCriticContPaper} presented in \secref{sec:hrl}.
Applying the concepts introduced in \secref{sec:hrl} is not sufficient for successfully learning \gls{etc} strategies. This is due to the special nature of the \gls{etc} problem. When using the algorithm in a standard, periodic control setting, both options coincide to sampling a continuous action from the respective intra option policy and applying it to the system. On the contrary, in \gls{etc}, choosing option 0, \ie the \gls{zoh}, directly fixes the action and, thus, introduces a great difference between the capabilities of the options. Simply put, in \gls{etc}, the two options cannot compensate for each other as only option 1 is capable of changing the action applied to the system. To account for this difference, we next propose several modifications to the original algorithm, mainly focused on stabilizing the learning process and increasing exploration on the options level. 
%The proposed algorithm allows to successfully learn \gls{etc} strategies from scratch through joint optimization.\db{Would leave out the last sentence}

Due to the different capabilities of the two options in \gls{etc}, learning the policy over options is very sensitive. However, in the original \gls{ppoc} framework, the authors propose to only use \gls{ppo} for updating the intra option policy, while the policy over options is refined using vanilla policy gradient \eqref{eq:vanilla_grad_pol_op}. In contrast, we propose to also use the \gls{ppo} algorithm for updating the policy over options for two reasons. First, the learning process is more sensitive due to the limited action of the \gls{zoh} in case of no communication. 
Second, as the two policies influence and affect each other, as can be seen in~\eqref{eq:conv_flat}, restricting the update process for both of the policies enhances the overall performance and stabilizes the learning process. Let $\theta_\mu$ denote the parameters of the policy over options, subject to optimization, and $\mu'=\mu(\theta_\mu)$ the new policy, while $\mu=\mu(\theta_{\mu_{old}})$ represents the old one. Using \gls{ppo} to update the policy over options results in
\begin{equation}
\begin{split}
L(\theta_\mu) &= R(\mu')-R(\mu)=Q(x_k,o(\mu'))-Q(x_k,o(\mu)) \\
&=r(x_k,o(\mu'))+\gamma V^{\mu}(x_{k+1}) - V^{\mu}(x_k)  \\
&= A^{\mu}(x_k,u^{\mu'}) \approx \frac{\mu'(o|x_k)}{\mu(o|x_k)} A^{\mu}(x_k,o^{\mu}) \text{ ,}
\end{split} 
\end{equation}
where $V$ is the value function and defined as $V(x)=\sum_{\tilde{o}}^{} \mu(\tilde{o}|x) Q(x,\tilde{o})$. 
Thus, exploiting the \gls{ppo} algorithm, the gradient is given by
\begin{equation}
\begin{split}
\frac{\partial L(\theta_\mu)}{\partial \theta_\mu} &= E [\frac{\partial}{\partial \theta_\mu} \min[\frac{\mu'(o|x)}{\mu(o|x)} A^{\mu}(x,o^{\mu}), \\ &\text{clip}(\frac{\mu'(o|x)}{\mu(o|x)},1-\epsilon,1+\epsilon) A^{\mu}(x,o^{\mu})]] \text{ .}
\end{split}
\end{equation}

For calculating the advantage function in this case, there are two possibilities:
\begin{enumerate}
\item $A^{\mu}(x,o^{\mu}) = Q(x,o) - \max_{o'} Q(x,o') \text{ ;}$
\item $A^{\mu}(x,o^{\mu}) = Q(x,o) - \sum_{\tilde{o}}^{} \mu_{\text{old}}(\tilde{o}|x) Q(x,\tilde{o}) \text{ .}$
\end{enumerate}
The first possibility represents a greedy approach as the baseline is the maximum Q-value possible, whereas the second one represents the expected Q-value under the old parameters. In preliminary experiments, the first version performed better and is, therefore, used herein.

The discrepancy in the capabilities of the options also affects the exploration process. While any continuous control input can be applied in the case of communication (\ie option 1), option 0 is extremely limited. The algorithm might tend to only choose option 1 as, especially at the beginning of the learning process, the \gls{zoh} will likely result in no improvements of the reward. Hence, we introduce an entropy term in the optimization algorithm. The entropy scheduling ensures that there is enough exploration for the policy over options, which handles the communication decision. The gradient for the policy over options, therefore, equates to 
\begin{equation}
\begin{split}
&\frac{\partial L(\theta_{\mu'})}{\partial \theta_{\mu'}} = \frac{\partial}{\partial \theta_{\mu'}} \mathbb{E} [\min[\frac{\mu'(o|x)}{\mu(o|x)} A^{\mu}(x,o) , \text{clip}(\frac{\mu'(o|x)}{\mu(o|x)}, \\
&1-\epsilon,1+\epsilon) A^{\mu}(x,o)] + \tau \text{log}(\mu'(o|x)) \mu'(o|x)] \text{,}
\end{split}
\end{equation}
where $\tau$ represents the entropy regularization coefficient. Over time, the entropy regularization is reduced as enough exploration has been conducted and, therefore, a rather exploitative behavior is preferred.

Considering the optimization objectives of the original \gls{ppoc} algorithm reveals that the gradients of the policy over options, as well as the termination function, effectively optimize the same objective (see  \eqref{eq:vanilla_grad_pol_op}, \eqref{eq:vanilla_grad_term}). The policy over options is supposed to choose the option with the highest Q-value, and the termination function should terminate the current option when another option has a higher estimated Q-value. As this is the same goal, we remove the termination function (\ie $\beta(x) \equiv 1$). In this new setting, one can also interpret termination as the policy over options deciding to choose another option. This modification simplifies the learning process, as only two policies have to be optimized. It further clearly establishes the link to the \gls{etc} problem formulation. The discrete decision of the policy over options coincides with the triggering law, while the intra option policy represents the control law. 

The resulting algorithm for learning the hierarchical control policy is presented in \algref{alg:learn_etc}. We use \gls{nn} policies to represent the policy over options, the intra option policy, as well as to approximate the Q-function. Details on the network structures are provided in \appref{sec:append_parametrization}.

Due to the \gls{zoh}, we have to include the last control action applied to the system in the state to keep the properties of a Markov decision process. Therefore, we define
%$\tilde{x}[k] = \begin{pmatrix} x[k] & u_\text{ac}[k-1] \end{pmatrix}^\transp$.
$\tilde{x}[k] = (x[k],~u_\text{ac}[k-1])^\transp$.

%Using our proposed algorithm for learning \gls{etc} from data results in better performance compared to simply using the original \gls{ppoc} framework. 
%\st{Should we illustrate this with numerical results?  This would emphasize that the modifications you have done are important, so it is more than "just" applying an existing framework to your problem.}

\begin{comment}
If not stated differently, the entropy coefficient $\tau$ is always divided by $10$ after 1000 epochs passed.
\end{comment}



\begin{algorithm}
\caption{Hierarchical RL for \gls{etc}}
\begin{algorithmic}[1]
  \small
  \State Initialize Clipping $\epsilon$ and Entropy Regularization $\tau$
  \State Inititalize Q-Network $Q(x,o)$
  \State Initialize Policy over options network $\mu(o|x)$
  \State Initialize Intra option policy network $\pi_o(u|x)$
  \For{number of epochs}
  	\State $Q' \leftarrow Q$
  	\State $\mu' \leftarrow \mu$
  	\State $\pi_o' \leftarrow \pi_o$
  	\State Sample $(x,o,u)$-Transitions using current $\mu$, $\pi$
  	\State Use GAE (\cite{schulman2015GAE}) to calculate $A^{\pi}(x,o,u)$
  	\For{number of optimizer iterations}
  		\For{number of options, $o=0,1,2,...$}
  			\State Sample batch
  			\State $A^{\mu}(x,o) = Q'(x,o) - \max_{\tilde{o}} Q'(x,\tilde{o})$
  			\State $L_1(\theta_{\mu'}) = \mathbb{E} [\min[\frac{\mu'(o|x)}{\mu(o|x)} A^{\mu}(x,o) , \text{clip}(\frac{\mu'(o|x)}{\mu(o|x)},$ \phantom a \phantom a \phantom a \phantom a \phantom a \phantom a \phantom a \phantom a \phantom a $1-\epsilon,1+\epsilon) A^{\mu}(x,o)] + \tau \text{log}(\mu'(o|x)) \mu'(o|x)]$ 
  			\State $L_2(\theta_{\pi'}) = \mathbb{E} [\min[\frac{\pi_o'(u|x)}{\pi_o(u|x)} A^{\pi}(x,o,u) , \text{clip}(\frac{\pi_o'(u|x)}{\pi_o(u|x)}, $ \phantom a \phantom a \phantom a \phantom a \phantom a \phantom a \phantom a \phantom . $1-\epsilon,1+\epsilon) A^{\pi}(x,o,u)]]$
  			\State $L_3(\theta_{Q'}) = \mathbb{E} [(Q'-(Q(x,o)+A^{\pi}(x,o,u)))^2]$
  			\State $\theta_{\mu'} \leftarrow \theta_{\mu'} + \alpha_{\theta_\mu} \frac{\partial L_1(\theta_{\mu'})}{\partial \theta_{\mu'}}$
  			\State $\theta_{\pi'} \leftarrow \theta_{\pi'} + \alpha_{\theta_{\pi'}} \frac{\partial L_2(\theta_{\pi'})}{\partial \theta_{\pi'}}$
  			\State $\theta_{Q'} \leftarrow \theta_{Q'} - \alpha_{\theta_{Q'}} \frac{\partial L_3(\theta_{Q'})}{\partial \theta_{Q'}}$
  		\EndFor 
  	\EndFor
  	\Comment{One potential implementation of the entropy scheduling is shown below}
  	\If {epoch \% 1000==0}
  		\State $\tau=\tau /10$
  	\EndIf
  \EndFor
\end{algorithmic}
\label{alg:learn_etc}
\end{algorithm}




==> chapters_old/5_ProofOfConceptChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TeX root = ../report.tex

\chapter{Proof of Concept}
\label{chp:ProofOfConcept}

In the following chapter, a proof of concept for the previously presented ideas and algorithms is presented. We apply the concepts to a slightly modified version of the OpenAI Gym Pendulum environment \cite{openaigym}.

\section{Parametrization of the proposed Algorithm}
\label{sec:parametrization}

Before proceeding, we first provide insights on how we implement the major components needed for the proposed algorithm (\algref{alg:learn_etc}). We use the same design choices for all the results presented from here on.

As explained in \secref{sec:leveragingrl_etc}, our implementation is based on three main components, the policy over options $\mu(o|\tilde{x})$, the intra option policy $\pi(u|\tilde{x},o)$, and the Q-function $Q(\tilde{x},u)$. \figref{fig:arch_pol_op}, \figref{fig:arch_intra_op}, and \figref{fig:arch_q_fct} show the standard implementations of the respective components for the case of using 2 options. \figref{fig:arch_intra_op} illustrates that for the case of performing the \gls{zoh}, \ie option 0, the intra option policy does not have to be evaluated. Thus, computational resources can be saved in the forward, as well as the backward pass. For implementing the \gls{nn} estimator of the Q-function (see \figref{fig:arch_q_fct}), we decided to split the estimates for option 0 and option 1 already before the first hidden layer. The reason for this choice is that as the two options are very different, we also expect very different Q-values for the two options, although being in the same state $\tilde{x}$. This is due to the fact that option 0 is limited to the \gls{zoh}, while option 1 can basically apply any action, depending on the intra option policy. For the same reasons, we arrive at the design choice for the policy over options (see \figref{fig:arch_pol_op}).

For the stability verification and retraining procedure, we apply the following modifications to the previously presented implementation. Instead of using the \gls{tanh} activation function, we apply the \gls{relu} activation. The number of hidden neurons is decreased from 64 to 32. This is due to the fact that at the core of the verification algorithm, we run a modified version of the Simplex algorithm, which simply runs faster if less neurons are used. Further, instead of using the softmax activation function for the policy over options, we calculate $Z=\zeta_0-\zeta_1$. If $Z>0$, this corresponds to performing the \gls{zoh} and choosing option 0, otherwise we use option 1. That way, we achieve deterministic behavior of the policy over options and avoid using the softmax activation function. Moreover, this deterministic decision is compatible with the stochastic case, as $Z=0$ equals to $\mu(o=0|\tilde{x})=\mu(o=1|\tilde{x})=\SI{50}{\percent}$, and $Z>0$ corresponds to $\mu(o=0|\tilde{x})>\mu(o=1|\tilde{x})$.

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/POC/NN/pol_op.png}
\caption{Exemplary illustration of the parametrization of the policy over options. In this specific implementation, each hidden layer consists of 64 neurons, and the \gls{tanh} and softmax activation functions are used. The variables $\zeta_0$ and $\zeta_1$ represent intermediate values.}
\label{fig:arch_pol_op}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/POC/NN/intra_opt.png}
\caption{Exemplary illustration of the parametrization of the intra option policy. In this specific implementation, each hidden layer consists of 64 neurons, and the \gls{tanh} activation function is used.}
\label{fig:arch_intra_op}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/POC/NN/q_fct.png}
\caption{Exemplary illustration of the parametrization of the Q-function estimator. In this specific implementation, each hidden layer consists of 64 neurons, and the \gls{tanh} activation function is used.}
\label{fig:arch_q_fct}
\end{figure}

\section{Introducing the Simulation Environment}

The equations of motion, in discrete-time, of the pendulum, are given by
\begin{equation}
\begin{split}
\theta[k+1] &= \theta[k] + \Delta T \dot{\theta}[k] + v_\theta[k]  \\
\dot{\theta}[k+1] &= \dot{\theta}[k] + \Delta T \ddot{\theta}[k] + v_{\dot{\theta}}[k]\\ 
&=\dot{\theta}[k] + \Delta T (\frac{-3g}{2l} \sin(\theta[k] + \pi ) + \frac{3}{ml^2} u[k]) + v_{\dot{\theta}}[k] \text{ ,}
\end{split}
\end{equation}

where $\theta$ represents the angle, $\dot{\theta}$ the angular velocity, $v$ the process noise, $u$ the control action, $\Delta T$ the time discretization, $m$ and $l$ the mass and the length of the pendulum, and $g$ the gravitational constant. The process noise is drawn from a standard normal distribution, scaled by $10^{-4}$. In addition, we add measurement noise $w$ of the same magnitude. Thus, the measurements are $\hat{\theta}[k]=\theta[k]+w_{\theta}[k]$, and $\hat{\dot{\theta}}[k]=\dot{\theta}[k]+w_{\dot{\theta}}[k]$. Those equations represent a forward integration of the nonlinear dynamics of the system in continuous time, and they do not include any damping.

If not stated differently, the goal is to stabilize the pendulum on top, \ie to keep the angle around $\theta=\SI{0}{\degree}$. When linearizing the original nonlinear, continuous-time, differential equation around this equilibrium, we arrive at $\ddot{\theta}=\frac{3g}{2l}\theta+\frac{3}{ml^2}u$. Using the values from the original environment, we get a time constant of the linearized system of $\tau=\sqrt{\frac{2l}{3g}} \approx \SI{0.26}{\second}$. 

Therefore, using a sampling rate of \SI{20}{\Hz}, as specified in the original implementation, should be sufficient for reliable and stable feedback control. This choice is rather on the lower end of the rule of thumb in feedback control that the sampling rate should be 5-10 times faster than the system dynamics. Thus, achieving huge communication savings is already a challenging problem.

\section{Learning Event-triggered Control}

In the following, we present results on learning \gls{et} control from scratch on the pendulum, using \algref{alg:learn_etc} and \eqref{eq:zoh_gen_opt}.

The control cost at each timestep is given by 
\begin{equation}
\label{eq:ctrl_cost}
J_{\text{ctrl}}[k]=1.0 \theta[k] + 0.1 \dot{\theta}[k] + 0.1 u[k] \text{ ,}
\end{equation}
and the overall cost is given by \eqref{eq:cost_fct}, using $\gamma=0.99$. The associated reward $R$ is obtained through $R=-J$. Those parameters are the same as in the standard OpenAI Gym implementation. We only increased the penalization on the control input from 0.001 to 0.1 to prevent the controller from being too aggressive.

\begin{figure}
\centering
\includegraphics[width=0.85\textwidth]{img/POC/stabilize/Learning_progress.png}
\caption{Illustration of the evolution of $R=-J$ during training, depending on the communication penalty $\lambda$. For higher values of $\lambda$, the final reward is bigger. It also seems that the higher $\lambda$, \ie the more resource-efficient one wants to be, the slower the training process.}
\label{fig:train_speed_top}
\end{figure}

\figref{fig:train_speed_top} illustrates the training progress for different values of the communication penalization factor $\lambda$. For higher values of $\lambda$, the overall reward $R$ is lower as the communication penalty is higher and increasing the communication savings negatively affects the control performance. Moreover, it also seems that the number of epochs it takes, until the training runs converge is larger for larger values of $\lambda$. This might reflect the fact that it is tougher to come up with a very resource-efficient control and communication strategy than with a policy that does not have to save as much communication due to a lower value of $\lambda$. While for $\lambda=0$, the average communication savings are around \SI{5}{\percent} (see \figref{fig:5percent_pend_top}), $\lambda=5.0$ results in communication savings up to around \SI{90}{\percent} (see \figref{fig:5percent_pend_top}). Those results are in line with the findings presented in \cite{BaumannRL}.

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/stabilize/eval_model_param-5_commpen5-0_seed200_exemplary_rollout_improved.eps}
	\caption{Illustration of the performance of a learned communication and control policy that saves about \SI{5}{\percent} of communication.}
	\label{fig:5percent_pend_top}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/stabilize/eval_model_param-5_commpen5-0_seed999_exemplary_rollout_improved.eps}
	\caption{Illustration of the performance of a learned communication and control policy that saves about \SI{90}{\percent} of communication.}
	\label{fig:90percent_pend_top}
	\end{subfigure}
\end{subfigure}
\caption{Exemplary rollouts of learned policies that save different amounts of communication. The agents are trained using the proposed algorithm.}
\label{fig:comm_savings_pend_top}
\end{figure}

\newpage

Since this task is linear, we can also compare our results to other well-known \gls{etc} algorithms. We linearize the pendulum around the upper equilibrium point and compare our approach to
\begin{itemize}
\item \textbf{LQR}: \\ $u[k] = K x[k] \Rightarrow \delta[k]=1 \text{ } \forall k \text{ ,}$
\item \textbf{LQR random skip}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \nu>\xi  \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $  
\item \textbf{state triggering 2 norm}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{x[k]}_2>\xi    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\item \textbf{output based triggering} \cite{6069816}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{K\hat{x}[k]-Kx[k]}_2>\xi \norm{Kx[k]}_2    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\item \textbf{state diff triggering} \cite{tabuada2007event}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{\hat{x}[k]-x[k]}_2>\xi \norm{x[k]}_2    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\end{itemize}
where $\hat{x}[k]$ represents the state at the last triggering instance and $\xi$ a threshold variable. I.e., by adjusting this threshold value, the triggering condition is altered, and therefore, the communication savings $\Gamma$ change. The random variable $\nu$, used in LQR random skip, is uniformly sampled from the interval $[0,1]$.

The gain matrix K is always chosen from the same LQR design with weigh matrixes $Q=\text{diag}([1.0,0.1])$ and $R=\begin{bmatrix} 0.1 \end{bmatrix}.$ This design choice again coincides with the parameters given by the standard OpenAI Gym implementation. Only the penalization on the control input has been increased from $0.001$ to $0.1$, to put more emphasis on a smooth control signal and to avoid to saturate the available input. The choice also ensures that the controller optimizes the same objective as the \gls{rl} agents \eqref{eq:ctrl_cost}.

\figref{fig:pareto_pend_top} shows the performance of the introduced event-triggering laws, together with the performance from our data-based \gls{rl} algorithm. As can be seen, for the classical approaches, only communication savings up to about \SI{80}{\percent} are possible, whereas our algorithm can come up with policies that can save up to \SI{90}{\percent}. However, for intermediate communication savings, the classical methods usually outperform our learning-based approach. This might be due to the fact that at these intermediate saving rates, there exist many local optima, and thus, our learning-based approach is prone to finding those suboptimal solutions. Nevertheless, the rewards of the classical approaches and our algorithm are in the same order of magnitude. In contrast, the learning approach introduced in \cite{BaumannRL} was also able to achieve communication savings of \SI{90}{\percent}, but was outperformed by orders of magnitude on intermediate communication savings.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{img/POC/stabilize/pareto.eps}
\caption{Illustration of the magnitude of $R_\text{ctrl}=-J_\text{ctrl}$ vs. the communication savings $\Gamma$ for various \gls{etc} strategies. For the learning agents, trained through the proposed algorithm, the best-trained policies have been selected. The mean and standard deviation are obtained by performing 10 rollouts with each of the policies.}
\label{fig:pareto_pend_top}
\end{figure}

The code for learning \gls{etc} from scratch and evaluating the models can be found at the git-amd server \footnote{\url{https://git-amd.tuebingen.mpg.de/nfunk/ppoc_off_tryout}}.

\newpage

\section{Stability Analysis and Retraining}

In the following section, we demonstrate how to show stability for \gls{nn} policies in the pendulum environment. The goal is to stabilize the pendulum in an upright position. Thus, we can obtain a linear system by linearizing the equations around the upper equilibrium point $\theta=\SI{0}{\degree}$ and $\dot{\theta}=\SI{0}{\degree / \second}$. The conversion from continuous to discrete-time is done using the matrix exponential method. 

For all of the following experiments, in line with Definition \ref{def:stability_def}, we define the safe state space ($\mathcal{O}$) to capture ranges of $\theta \in [\SI{-2.5}{\degree},\SI{2.5}{\degree}]$ and $\dot{\theta} \in [\SI{-5}{\degree / \second},\SI{5}{\degree / \second}]$. 

Usually, the state of the pendulum environment that is fed into the \gls{nn} to obtain the control action, is given by $x[k]=\begin{pmatrix} \cos(\theta[k]) & \sin(\theta[k]) & \dot{\theta}[k] \end{pmatrix}^T$. However, since for the stability verification algorithm we need to express the output of the \gls{nn} policy in terms of the variables of the system dynamics, \ie $\theta[k]$ and $\dot{\theta}[k]$, and can neither use the nonlinear sine nor the cosine function, we also linearize the state of the environment around the equilibrium which results in $x[k] \approx \begin{pmatrix} 1.0 & \theta[k] & \dot{\theta}[k] \end{pmatrix}^T$.

\subsection{Stability Analysis and Retraining - Periodic Control}

First, results for the stability analysis of \gls{nn} policies will be presented for the case when no resource constraints are active. Thus, we consider the setting of having one single \gls{nn} policy that simply outputs the action given the state.

For checking the stability of any \gls{nn} policy, one has to put them into the stability checking algorithm (\algref{alg:check_stab}). If the algorithm returns that there is not one single point violating the constraints, then this policy, in combination with the system dynamics, is considered to be stable. However, as \gls{nn} policies have many parameters and, therefore, also many degrees of freedom, it is obvious that this stability check is fulfilled very rarely. As shown in the previous chapter (\secref{sec:retrain_periodic}), the results from the stability analysis can be exploited to refine existing \gls{nn} control policies such that they fulfill the desired stability properties. This process is illustrated in \figref{fig:retrain_periodic_pendulum}, where a randomly initialized \gls{nn} policy is refined using \algref{alg:refine_pol}. After running the algorithm for 16 epochs, we arrive at a stable controller. Interestingly, although the stability retraining was only designed for an angular range of $\theta \in [\SI{-2.5}{\degree},\SI{2.5}{\degree}]$, the refined control policy also yields stable results when starting outside of this region.

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/only_comm/eval_model_param0_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum with a randomly initialized policy, for the case of periodic control, without any event-trigger. Each color represents a different rollout.}
	\label{fig:retrain_periodic_pendulum_l}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/only_comm/eval_model_param16_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum after retraining the policy with \algref{alg:refine_pol} for 16 epochs. The pendulum is now stabilized successfully. Each color represents a different rollout.}
	\label{fig:retrain_periodic_pendulum_r}
	\end{subfigure}
\end{subfigure}
\caption{Effect of the retraining procedure presented in \algref{alg:refine_pol}, for the case of  periodic control. After refining the randomly initialized policy for 16 iterations, a guaranteed stable controller is obtained, which successfully stabilizes the pendulum. While the initial controller (\figref{fig:retrain_periodic_pendulum_l}) is unstable, as the pendulum falls down, after applying the retraining, the controller is stable and the pendulum is kept upright (\figref{fig:retrain_periodic_pendulum_r}).}
\label{fig:retrain_periodic_pendulum}
\end{figure}

\subsection{Stability Analysis and Retraining - Event-triggered Control}

When also adding the communication decision into the stability check, the complexity of the check and retraining procedure doubles. The reason lies in the fact that we have to compute the next state for both of the cases, \ie for communicating and for not communicating (see \algref{alg:check_stability_ET_rigorous}). Then, the policy over options has to be evaluated to know whether the next state is inside the stable set or not. 

The results of running the retraining procedure are shown in \figref{fig:retrain_et_pendulum}. As one can see, after retaining for 4 iterations, a guaranteed stable controller is obtained, which successfully stabilizes the pendulum while still saving communication. Again, although we only trained for an angular region between \SI{-2.5}{\degree} and \SI{2.5}{\degree}, as shown in \figref{fig:retrain_et_pendulum_stable}, the policy also yields a stabilizing performance when starting outside of this interval. Over 10 randomly started runs, the policy saves around \SI{70}{\percent} of communication. An exemplary rollout of this very resource-efficient and guaranteed stable control policy can be seen in \figref{fig:retrain_et_pendulum_rollout}. To ensure that the refined policy still saves communication, it is important to include the constraint to skip communication whenever possible. Otherwise, the retraining procedure results in a policy that is always communicating.

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/full/eval_model_param0_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum with an \gls{et} policy, after 500 optimization epochs. Each color represents a different rollout.}
	\label{fig:retrain_et_pendulum_unstable}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/full/eval_model_param4_angles.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum after retraining the policy with  \algref{alg:refine_pol} for 4 epochs. The pendulum is now stabilized successfully, while still saving communication. Each color represents a different rollout.}
	\label{fig:retrain_et_pendulum_stable}
	\end{subfigure}
\end{subfigure}
\caption{Effect of the retraining procedure presented in \algref{alg:refine_pol ET}, for the case of event-triggered control. While the initial policy is unstable (\figref{fig:retrain_et_pendulum_unstable}), after refining policy for 4 iterations, a guaranteed stable controller is obtained which successfully stabilizes the pendulum and still saves about \SI{70}{\percent} of communication (\figref{fig:retrain_et_pendulum_stable}).}
\label{fig:retrain_et_pendulum}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1.0\textwidth]{img/Marabou/full/eval_model_param4_exemplary_rollout.eps}
\caption{Illustration of an exemplary rollout of the same policy, as shown in \figref{fig:retrain_et_pendulum_stable}.}
\label{fig:retrain_et_pendulum_rollout}
\end{figure}

The code for the stability verification algorithm and retraining procedure can be accessed at \footnote{\url{https://git-amd.tuebingen.mpg.de/nfunk/ppoc_off_tryout}}.

\section{Learning Hierarchical, Periodic Control}

The application of our derived hierarchical \gls{rl} algorithm is not limited to the case of \gls{etc} only. One can also use this algorithm and equip both options with continuous control policies. In this short section, we provide results when both of the policies coincide with communication. The two options represent two different \glspl{nn} from which we can sample the actions. Further, we now consider the task of swingup and stabilization of the pendulum. We compare the results obtained by our algorithm with the original \gls{ppoc} implementation \cite{OptionCriticContPaper}, upon which we base our work. Choosing a hierarchical \gls{rl} framework is intuitive for this task as one could think of subdividing it into swingup and stabilization. 

\figref{fig:train_all_comparison} depicts the difference in the learning behavior between the \gls{ppoc} algorithm and our proposed approach. As can be seen in \figref{fig:training_all_comm_own}, the learning progress for our algorithm is way more stable compared to the \gls{ppoc} framework, see \figref{fig:training_all_comm_ppoc}. We think that the main reason for this gravely different behavior is that we also constrain the updates on the policy over options using PPO. One explanation, why this difference is so striking in the pendulum environment is that the reward changes gravely whenever the pendulum falls down. Therefore, using a rather smooth exploration strategy and limiting the updates for all of the policies involved, greatly stabilizes the learning process. A steady learning process is especially crucial in the \gls{et} setting, where the second option cannot compensate for anything but simply performs a \gls{zoh}. Thus, we think that our algorithm is better suited for \gls{etc}.

Nevertheless, the rollouts of the best performing policies, for both of the learning algorithms, result in comparable performance. Moreover, for both algorithms, only some of the policies exhibit the split behavior, \ie one option exclusively handling the swingup and the other one stabilizing the pendulum. 

\begin{figure}
\begin{subfigure}{1.0\textwidth}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/all_comm/own_algo.eps}
	\caption{Training progress for swingup and stabilization of the pendulum using our own algorithm and two fully functional options.}
	\label{fig:training_all_comm_own}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/POC/all_comm/ppoc.eps}
	\caption{Training progress for swingup and stabilization of the pendulum using the PPOC algorithm and two fully functional options.}
	\label{fig:training_all_comm_ppoc}
	\end{subfigure}
\end{subfigure}
\caption{Comparison of the learning progress for the two algorithms.}
\label{fig:train_all_comparison}
\end{figure}


==> chapters_old/6_HighdimensionalResultsChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section{Results in Simulation Environments}
\label{chp:ResultsHighdimensional}

To showcase the versatility of the presented algorithm, we apply it to low-dimensional and linear as well as high-dimensional and nonlinear systems.
%The main advantage of the presented algorithm compared to existing work lies in its versatility.
%The algorithm can, without any modification, be applied to low-dimensional and linear as well as high-dimensional and nonlinear systems.
%To demonstrate this, 
We first present results for the OpenAI Gym \cite{1606.01540} Pendulum environment.
This simple environment also allows us to compare the algorithm's performance to classical \gls{etc} approaches.
Next, we show its behavior in challenging nonlinear and high-dimensional MuJoCo \cite{todorov2012mujoco} environments.
%We are not aware of any other algorithm that can come up with \gls{etc} strategies through jointly optimizing communication and control in such challenging environments.

For all simulation experiments, we use two options as shown in \eqref{eq:zoh_gen_opt}. The reward is given by \eqref{eq:cost_fct}, where, if not stated differently, $R_{\text{ctrl}}[k]$ is the unmodified reward provided by the respective environment. For all the experiments, we use the environments' original sampling rate of \SI{20}{\Hz}.

We train all of the agents for 5000 epochs and store the model that achieves the highest reward. Each epoch consists of sampling 2048 $(s,o,a)$-transitions. For each communication penalty $\lambda$, we start 10 training runs with different seeds and report the performance of the best models. The \gls{nn} architectures are presented in~\appref{sec:append_parametrization}. The code that has been used to train the learning-based models and videos illustrating the results are available at \footnote{\label{cont}\scriptsize{\url{https://sites.google.com/view/learn-event-triggered-control}}}.
%\db{either write it the way you have it and have the url as part of the text, not as a footnote, or leave out the sentence, just have a footnote after the preceding sentence, and write in the footnote text that code is available at\ldots}

\subsection{Pendulum Environment}
\label{sec:poc}

In this rather simple environment, we consider the challenge of  stabilizing the inverted pendulum on top, already starting in an upright position. We use the reward function's original parameters, except for increasing the penalization on the control input from 0.001 to 0.1 to prevent the controller from being too aggressive.
%Calculating the time constant of the linearized system results in $\SI{0.26}{\second}$. Therefore, using the original sampling rate of \SI{20}{\Hz} should be sufficient for reliable and stable feedback control. This choice is rather on the lower end of the rule of thumb in feedback control that the sampling rate should be 5-10 times faster than the system dynamics. Thus, achieving huge communication savings is already a challenging problem.

For this task, it is straightforward to linearize the system dynamics around the equilibrium. This allows us to compare the results of the presented algorithm to other well-known \gls{etc} approaches. In particular, we compare our algorithm to 

{\scriptsize
\begin{itemize}
\item \textbf{LQR}: \\ $u[k] = K x[k] \Rightarrow \delta[k]=1 \text{ } \forall k \text{ ,}$
\item \textbf{LQR random skip}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \nu>\xi  \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $  
\item \textbf{state triggering 2 norm}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{x[k]}_2>\xi    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\item \textbf{output based triggering} \cite{6069816}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{K\hat{x}[k]-Kx[k]}_2>\xi \norm{Kx[k]}_2    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\item \textbf{state diff triggering} \cite{tabuada2007event}: \\ $u[k] = \begin{cases} K x[k] \Rightarrow \delta[k]=1, & \text{if } \norm{\hat{x}[k]-x[k]}_2>\xi \norm{x[k]}_2    \\
u[k-1] \Rightarrow \delta[k]=0, & \text{otherwise} \text{ ,} \end{cases} $
\end{itemize}
}
where $\hat{x}[k]$ represents the state at the last triggering instance and $\xi$ a threshold variable, adjusting the triggering condition. The random variable $\nu$ is uniformly sampled from the interval $[0,1]$. The gain matrix K is chosen from an LQR design where the weights are identical to the parameters of the reward function.

In \figref{fig:pareto_pend_top}, we show the performance of the introduced event-triggering laws and our data-based \gls{rl} algorithm. As can be seen, for the classical approaches, only communication savings up to about \SI{80}{\percent} are possible, whereas our algorithm finds policies that can save up to \SI{90}{\percent}. However, for intermediate communication savings, the classical methods usually outperform our learning-based approach. This might be caused by the algorithm getting stuck in local optima. Nevertheless, the rewards of the classical approaches and our algorithm are still in the same order of magnitude for the intermediate savings. This distinguishes the herein presented algorithm from the \gls{rl} framework proposed in~\cite{BaumannRL}, which also achieved communication savings of up to \SI{90}{\percent} in the pendulum environment, but was outperformed by orders of magnitudes for intermediate communication savings.

\begin{figure}
\centering
\includegraphics[width=\collen]{img/POC/stabilize/Figure_112.eps}
\caption{Illustration of the magnitude of the control reward $R_\text{ctrl}$ versus the communication savings $\Gamma$ for various \gls{etc} strategies and our learning approach for the task of stabilizing an inverted pendulum. The mean and standard deviation are obtained by performing 10 rollouts with each of the policies, and indicated by the grey lines. The vertical drops indicate when the policies become unstable, \ie fail to stabilize the pendulum. For intermediate communication savings, all the approaches show similar performance. Considering the maximum savings possible, the learning approach outperforms the others.}
\label{fig:pareto_pend_top}
\end{figure}

%The learning-based models have been obtained using communication penalties of $\lambda = 0.0, 0.5, 1.0, 5.0$ (from left to right).

\subsection{Results in high-dimensional, nonlinear Environments}
\label{ref:highdim}

We now focus on the nonlinear, high-dimensional MuJoCo Half-Cheetah (\figref{fig:cheetah_env}) and Ant (\figref{fig:ant_env}) environment, that cannot simply be linearized around certain equilibria points to yield linear system dynamics. In those challenging nonlinear environments, known approaches for \gls{etc} usually fail as the settings are too complex. To our knowledge, only \cite{BaumannRL} presents results in such environments. However, through separately learning control and communication. 
%This is the first work that jointly learns both in such challenging and especially high-dimensional settings.

In these environments, the reward $R_\text{ctrl}$ is mainly made up of the distance covered, but additionally includes a cost on the control action and contact forces. The goal of the optimization is to move the robotic agent as far as possible in the available time, given input and environmental constraints. Apart from the reward, we will also analyze the distance $d$ that the robotic agents cover during a rollout. We slightly modify the Ant environment by eliminating the restriction that limits the jump height of the center of mass of the Ant.


\begin{figure}
\begin{subfigure}{1.0\collen}
	\centering
	\begin{subfigure}[t]{0.475\textwidth}
	\centering
	\includegraphics[width=0.9\textwidth]{img/Highdim/envs/Cheetah.png}
	\caption{Half-Cheetah environment. Its observation space has 18 dimensions, and the action space 6.}
	\label{fig:cheetah_env}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.475\textwidth}
	\centering
	\includegraphics[width=0.9\textwidth]{img/Highdim/envs/Ant.png}
	\caption{Ant environment. Its observation space has 111 dimensions, and the action space 8.}
	\label{fig:ant_env}
	\end{subfigure} 
\end{subfigure}
\caption{The high-dimensional MuJoCo environments in which we train the learning agents.}
\label{fig:mujoco_envs}
\end{figure}  

\subsubsection{Half-Cheetah Environment}

%One obvious approach of a resource-aware policy in the Cheetah environment is to never communicate. In this environment, this results in the Cheetah standing still at its initial position. Indeed, the stability of the trainings, \ie the percentage of training runs that result in moving the Cheetah forward, is dependent on the communication penalization $\lambda$. Generally speaking, when increasing the value of $\lambda$, the percentage of successful training runs decreases as the option of never communicating becomes more and more attractive. Therefore, for high values of $\lambda$, the training runs naturally converge to not communicating at all. 

The red graph in \figref{fig:pareto_cheetah} illustrates the performance of policies trained using the presented algorithm. By increasing the value of $\lambda$, higher communication savings $\Gamma$ can be achieved while, on the other hand, the covered distance decreases. In this Half-Cheetah environment, we are capable of learning policies that can achieve up to \SI{80}{\percent} communication savings. In the figure, we showcase the performance of the nine best, out of ten rollouts with each policy. This is due to the fact that some of the policies exhibit one rollout where the Cheetah is flipped onto its back, resulting in a significantly decreased distance covered.

Interestingly, the communication savings have an impact on the gait, as shown in the accompanying video. More communication savings result in a rather jumpy policy; when the Cheetah is in the air, there is no need to communicate. One can see that for a low penalty on communication, the Cheetah's feet stay rather close to the ground, which also results in slightly faster progress. As shown in the red graph of \figref{fig:pareto_cheetah}, the standard deviation of the distance traveled is small, indicating that all the policies are robust and reliable. The training stability, \ie the percentage of training runs that result in moving the Cheetah forward, is dependent on the communication penalization $\lambda$. The percentage of successful training runs typically decreases as the value of $\lambda$ is increased, as the option of never communicating becomes more and more attractive. Therefore, for high values of $\lambda$, the training runs naturally converge to policies that do not communicate at all. This results in the Cheetah standing still at its initial position.

%\footnote{\url{https://youtu.be/emuPEFYkIYo}}\db{consider having a Google site or similar for all the videos (similar as for my CDC paper)} \footnotemark[\ref{cont}]

We also compare our algorithm's results with a baseline policy trained using the PPO algorithm. This baseline PPO policy only learns the control policy, while the communication strategy is fixed to always communicate. One possibility to achieve communication savings using this baseline policy is to randomly skip communication with a predefined probability. As can be seen in the blue graph in \figref{fig:pareto_cheetah} and the corresponding video, this rapidly decreases the performance. 
This emphasizes that it is crucial to optimize the control and communication strategy jointly. The models trained using our algorithm outperform the baselines. They are considerably more resource-efficient while the Cheetah still covers at least the same distance.
%The superiority of the joint optimization is further underlined by comparing the performance of our algorithm with the original \gls{ppo} baseline and the baseline under randomly skipping communication as can be obtained from the accompanying videos. As shown, the models trained using our algorithm outperform the baselines. They are considerably more resource-efficient while the Cheetah still covers at least the same distance.

As an additional benchmark, we implemented a modified version of the proposed algorithm that optimizes the control and communication strategy separately, in an alternating fashion. The performance of these agents is visualized through the black and purple graph in \figref{fig:pareto_cheetah}. To obtain the agents corresponding to the black and purple line, we switch between solely optimizing control and solely optimizing communication, every 25 respectively 100 epochs. As can be seen, the proposed joint optimization approach outperforms the separate optimization method. Considering low communication savings, the difference in performance is small. However, for high communication savings, it is significant. This highlights that especially for more difficult tasks, where it is crucial to finely adjust the two policies to each other, the joint optimization approach is superior. The experiments also illustrate that a higher frequency of alternation (black graph) results in better performance. Further increasing the frequency of alternation naturally converges to the joint optimization approach.

%\footnote{\url{https://youtu.be/Q3gbPoH9zLg}} 
% \footnotemark[\ref{cont}]
%\footnote{\url{https://youtu.be/eQrpg2s262M}} 
We additionally investigate the significance of the modifications detailed in \secref{sec:leveragingrl_etc}.
For this, we try to learn an \gls{et} controller using the original \gls{ppoc} implementation (see \secref{sec:hrl}). As shown in \figref{fig:pareto_cheetah}, for $\lambda=0.0$, the \gls{ppoc} algorithm finds a solution that saves a minimal amount of communication. However, for higher values of $\lambda$, e.g., 1.0, the \gls{ppoc} algorithm always results in a policy that never communicates, and therefore, the Cheetah does not progress at all. Thus, unlike our algorithm, the original \gls{ppoc} algorithm is incapable of arriving at \gls{et} controllers that reduce communication significantly, while still moving the Cheetah forward. This is probably due to the greedy optimization of the \gls{ppoc} algorithm. Further insights are provided in \appref{sec:hierarchical_period_ctrl}.

\begin{figure}
\centering
\includegraphics[width=1.0\collen]{img/Highdim/cheetah/Figure_113.eps}
\caption{Illustration of the performance of various agents. Depicted is the distance traveled by the Half-Cheetah $d$ versus the communication savings $\Gamma$. The shown mean and standard deviation are calculated from the nine best, out of ten rollouts, and illustrated in grey. The red line connects the results obtained from agents, trained using our algorithm. The blue line combines the rollouts of a PPO baseline policy, which saves communication by randomly skipping communication. The purple and black lines connect the results obtained from agents, trained using a modified version of our proposed algorithm. I.e., control and communication are optimized separately, in an alternating fashion. For the black line, the optimization is switched every 25 epochs; for the purple one, every 100 epochs. The herein presented joint optimization approach outperforms the others in terms of performance at intermediate communication savings as well as maximum savings possible.}
\label{fig:pareto_cheetah}
\end{figure}
%The models have been obtained using communication penalties of $\lambda= 0.5, 0.5, 1.0, 2.5, 2.5, 4.0$ (from left to right).

\subsubsection{Ant Environment}
%\db{I thought the plan was to outsource this part to the Appendix?}
\begin{comment}
\begin{figure}
\begin{subfigure}{1.0\collen}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
	\includegraphics[width=\textwidth]{img/Highdim/ant/progress/Figure_1.eps}
	%\input{img/Highdim/ant/progress/test.tex}
	\caption{Learning progress for $\lambda=0.0$}
	\label{fig:ant_learning_progress_0_0}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.225\textwidth}
	%\includegraphics[width=\textwidth]{img/Highdim/ant/progress/1_0.eps}
		\includegraphics[width=\textwidth]{img/Highdim/ant/progress/Figure_2.eps}
	\caption{Learning progress for $\lambda=1.0$}
	\label{fig:ant_learning_progress_1_0}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.225\textwidth}
	%\includegraphics[width=\textwidth]{img/Highdim/ant/progress/2_5.eps}
		\includegraphics[width=\textwidth]{img/Highdim/ant/progress/Figure_3.eps}
	\caption{Learning progress for $\lambda=2.5$}
	\label{fig:ant_learning_progress_2_5}
	\end{subfigure}
\end{subfigure}
\caption{Learning progress for the Ant, using different values of $\lambda$. 
% The y-axis represents the reward, \ie $R$.
}
\label{fig:ant_learning_progress}
\end{figure}
\end{comment}

When deploying the algorithm to the even higher-dimensional Ant environment, we obtain similar results.
\figref{fig:pareto_ant} shows the distance covered by the Ant versus the communication savings $\Gamma$ for models trained using the proposed algorithm. We again show the performance of the nine best, out of ten rollouts for each policy since some policies exhibit one rollout where the Ant is flipped onto its back, resulting in a significantly decreased distance covered. As can be seen from the plot, the most resource-aware control policies are capable of saving up to \SI{70}{\percent} of communication. The figure also illustrates that performance degrades if the communication savings increase. The policy saving \SI{70}{\percent} exhibits the largest standard deviation. Therefore, it is the least stable, but also the most resource-efficient policy. The corresponding video from rollouts with different penalizations underlines those findings and aligns with the results for the Half-Cheetah. When more communication is possible, the Ant's feet are kept rather close to the ground, which results in fast progress, and more reliability as the chances of flipping are minimized. When the penalization on communication is progressively increased, the gait changes towards a rather jumpy behavior. This allows for the most significant communication savings, as when the feet are in the air, no communication is needed. Nevertheless, compared to the results for the Cheetah, the changes in the gait behavior are less obvious. Considering the training process, again, if the resource constraints become very restrictive, the learning process becomes more difficult, and never communicating also becomes a local optimum. 
%\footnotemark[\ref{cont}]
%\footnote{\url{https://youtu.be/yrvYs5CG1c8}}

\begin{figure}
\centering
\includegraphics[width=1.0\collen]{img/Highdim/ant/Figure_113.eps}
\caption{Illustration of the agents' performance, trained using our proposed algorithm. Depicted is the distance covered by the Ant $d$ versus the communication savings. The shown mean and standard deviation are calculated from the nine best, out of ten rollouts, and illustrated in grey. At maximum, \SI{70}{\percent} of communication can be saved.}
\label{fig:pareto_ant}
\end{figure} 
%$\lambda=0.0,0.0,0.5,0.5,1.0,2.5.2.5$ (from left to right).

Compared to \cite{BaumannRL}, where the authors also try to learn an \gls{etc} strategy from data for the Ant environment, the proposed joint optimization achieves even higher communication savings with up to \SI{70}{\percent}, whereas~\cite{BaumannRL} only reported savings of up to \SI{60}{\percent} for their separate optimization approach.


==> chapters_old/7_HardwareResultsChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section{Results on Hardware}
\label{chp:HardwareResults}

%\db{I would start here saying that in general it is difficult to use RL on hardware due to sample inefficiency. Just to highlight that these are impressive results.}
While many deep \gls{rl} methods have shown good performance in simulation environments, there are only few examples where the learned policies are actually deployed on real hardware. 
This is mainly due to the sample inefficiency of those algorithms or insufficient simulation to reality transfer.
% Mainly since the approaches are not very sample efficient. 
In this section, we present the results of using our learning algorithm on real hardware, namely, the Apollo robot shown in \figref{fig:hw_apollo_cup}. 

In contrast to the previous simulation experiments, which provide perfect communication and no delays, we now consider real experimental conditions with noise, delays, and potential packet losses. 
The experimental setup is as follows: the sensory information, \ie Apollo's joint configuration, is communicated to the learning agent running on a computer. The agent then decides whether or not to communicate, and, depending on that decision, eventually sends new control commands to the robot. We use a base sampling time of $\SI{20}{\hertz}$. Further details on the setup can be found in \appref{sec:supp_material_robot_exp}.

%We present experiments on \gls{etc} of Apollo's right arm which consists of 6 joints. For simulating the robot, we use the simulation laboratory (SL) framework \cite{SL__2009}. Further details on Apollo and the software setup can be found in \appref{sec:supp_material_robot_exp}. Videos of the experiments are available at \footnotemark[\ref{cont}].

\begin{comment}
% I think that this picture is not needed
\begin{figure}
\centering
\includegraphics[width=1.0\collen]{img/HW/apollo.JPG}
\caption{Apollo robot platform which is used to conduct the hardware experiments.}
\label{fig:hw_apollo}
\end{figure}
\end{comment}

\subsection{Problem Definition and Setup}
\label{sec:apollo_setup_definition}

To demonstrate the feasibility of the introduced framework, we employ a real-time position controller for the end-effector of Apollo's right arm with 6 \gls{dof}. The controller that is to be learned operates in the cartesian space. The goal is to reach a desired position as accurately as possible under resource constraints, \ie trying to communicate as efficiently as possible. The learning agent's output is a desired reference velocity in the task space of the end-effector,
%$u[k]=v_{\text{ref}}[k]=\begin{pmatrix}v_x[k] & v_y[k] & v_z[k] \end{pmatrix}^\transp$.
$u[k]=v_{\text{ref}}[k]=(v_x[k],~v_y[k],~v_z[k])^\transp$.

As the input to the robot has to be with respect to the individual joints, while the learning algorithm's output is defined in task space, the procedure is as follows. The learning algorithm outputs velocities in task space, which are then mapped to the corresponding commands in joint space through inverse kinematics. We use the Pinocchio library~\cite{carpentier2019pinocchio} for this step. The process of computing the target velocity in joint space is iterative and affected by the current robot configuration. It is not guaranteed that the desired velocity can be reached accurately. Once the velocities in joint space are computed, they are applied until the next instance of communication. In the beginning, the desired velocity is reached quite accurately. Considering a longer horizon, it is obvious that constant joint velocities do not coincide with a constant velocity in task space. Therefore, over time, the discrepancy between the desired and the actual velocity increases as there is no recomputation until the next instance of communication.

Since the learning agent only operates in the task space, the state which is fed to the agent is 
%$\tilde{x}[k] = \begin{pmatrix} \dot{x}_\text{ef}[k] &  x_{\text{ef}}[k] & x_{\text{ref}}[k] - x_{\text{ef}}[k] & u_\text{ac}[k-1] \end{pmatrix}^\transp$,
$\tilde{x}[k] = (\dot{x}_\text{ef}[k],~x_{\text{ef}}[k],~ x_{\text{ref}}[k] - x_{\text{ef}}[k],~u_\text{ac}[k-1])^\transp$, 
where $x_\text{ef}$ denotes end-effector position and $x_\text{ref}$ denotes the desired reference position that is to be reached, in cartesian coordinates. Thus, no joint information is available to the learning agent, which makes the setting partially observable.

In the settings in \secref{ref:highdim}, the steady-state solution is applying a sequence of control inputs to achieve a constant movement of the agent. However, for this task, once the end-effector is close to the reference, it is desirable to apply a zero action to hold its position. As it is unlikely that a \gls{nn} policy outputs exactly zero, we exploit our approach's hierarchical nature and simply define a third option ($o_2$) that corresponds to setting the control input to zero. Hence, for the hardware experiments, unlike presented in \eqref{eq:zoh_gen_opt}, we consider three options: 
%\\
%Options $o_0$ and $o_1$ as in~\eqref{eq:zoh_gen_opt} and option $o_2$, which corresponds to communicating ($\delta[k]=1$) and applying zero input, \ie $u_\text{ac}[k]=\begin{pmatrix}0 & 0 & 0 \end{pmatrix}^\transp$.
\begin{equation} \label{eq:hw_opt}
u_{\text{ac}}[k] = \begin{cases} u_{\text{ac}}[k-1], & \text{if } \delta[k] = 0 \text{, } o=o_0  \\
u_{\text{ag}}[k]=\pi_{o_1}(u|x), & \text{if } \delta[k] = 1 \text{, } o=o_1 \\
 u_{\text{ag}}[k]=\begin{pmatrix}0 & 0 & 0 \end{pmatrix}^\transp, & \text{if } \delta[k] = 1 \text{, } o=o_2
\text{ .}
\end{cases}
\end{equation}

\begin{comment}
\begin{itemize}
\item Option 0 ($o_0$) corresponds to no communication ($\delta[k]=0$) and performing the \gls{zoh};
\item Option 1 ($o_1$) corresponds to communicating ($\delta[k]=1$) and applying the control action output by the \gls{nn} policy;
\item Option 2 ($o_2$) corresponds to communicating ($\delta[k]=1$) and applying the zero action, \ie $u[k]=\begin{pmatrix}0 & 0 & 0 \end{pmatrix}^\transp \text{ .}$
\end{itemize}
\end{comment}

To obtain the results presented in the next sections, we first train the learning algorithm in simulation using the simulation laboratory (SL) framework \cite{SL__2009}. Then, we deploy the learned policies on the real robot. For the transfer from simulation to reality, no additional adjustments are performed.

\subsection{Dynamic Reference Position Tracking}
\label{sec:dynamic_reaching}

At first, we describe the performance of resource-aware agents trained for reaching a dynamic reference position. I.e., putting the end-effector close to a cup (\cf \figref{fig:hw_apollo_cup}) such that it could be grabbed. The cup's position is estimated using the Vicon system and included in the sensory information.

\begin{figure}
\centering
\includegraphics[width=0.6\collen]{img/HW/exemplary_cup_clipped_rev_1.png}
\caption{Illustration of the hardware experiment where the goal is to place Apollo's hand close to the cup. The cup's position is estimated using the Vicon system.}
\label{fig:hw_apollo_cup}
\end{figure}

During training, we choose a random initial position of the robot arm and a random reference position (representing the cup) inside the interval 
%$\begin{pmatrix} [-0.2, 0.5] & [0.55, 0.9] & [-0.15, 0.45] \end{pmatrix}^\transp \SI{}{\meter}$,
$([-0.2, 0.5],~[0.55, 0.9],~[-0.15, 0.45])^\transp\SI{}{\meter}$, 
for each trajectory. At each simulated timestep, the reference position is reset to another randomly sampled point inside this interval with probability \SI{1}{\percent}. This procedure should already account for the fact that during the evaluation on the real system, the reference will change dynamically. 

% We present the hardware results that use a model which has been trained for 2250 epochs, in simulation, using a communication penalty of $\lambda=0.1$. 
The policies, whose results are presented in the following, have been trained for \num{2250} epochs in simulation with a communication penalty of $\lambda=0.1$.
To incentivize reaching the final position more accurately, we added an inverse term to the reward function $R$, which is thus given by $R = \sum_{k=0}^N \gamma^k (R_{\text{ctrl}}[k] + R_{\text{comm}}[k]) = \sum_{k=0}^N \gamma^k (-3(0.01 {\norm{u[k]}_2}^2 + 10 {\norm{x_{\text{ref}}[k] - x_{\text{ef}}[k]}_2}^2 + 0.01 {\norm{\dot{x}_\text{ef}[k]}_2}^2   + \lambda \delta[k]) + \frac{5}{{\norm{x_{\text{ref}}[k] - x_{\text{ef}}[k]}_2}^2})$.
% This helped to reach the end position significantly more accurately as it increases the incentive to be more precise. 
%The reward is given by 

\begin{figure}
\centering
\includegraphics[height=0.9\textheight,keepaspectratio,width=\collen]{img/HW/final_normal.eps}
\caption{Exemplary rollout of a policy trained for the task of reaching a dynamic reference position with Apollo's right hand, see \figref{fig:hw_apollo_cup}. The reference (\ie the cup's position) is provided by the Vicon system. During the rollout, the policy saves $85\%$ of communication, while the reference is still tracked reliably. This performance is consistent among various runs.}
\label{fig:hw_rollout_dyn}
\end{figure}
%\protect\url{https://youtu.be/-Bcq_PSaITc}.
%Video available at \protect \footnotemark[\ref{cont}].

In \figref{fig:hw_rollout_dyn}, we depict an exemplary rollout of the model while tracking the reference signal provided by the Vicon system. It is striking that $85\%$ of communication can be saved while still reaching the dynamic desired reference reliably. As can be seen, the reference signal is sometimes slightly disturbed. However, although only trained in simulation without such nonidealities, the learning agent is robust to these disturbances. Thus, we conclude that we did not overfit and that our problem formulation and implementation results in a stable and robust simulation to reality transfer.
%we can successfully transfer obtained knowledge from simulation to the real robot. 
%In general, we found that our problem formulation and implementation results in a stable and robust simulation to reality transfer. 
The corresponding video illustrates the responsiveness of the final policy and confirms the low tracking error. The learned controller drives the hand close enough to the cup such that it can be grabbed.
%\footnote{\protect\url{https://youtu.be/-Bcq_PSaITc}}

\subsection{Obstacle Avoidance}

To further illustrate our learning algorithm's capabilities, we increase the difficulty and demonstrate the resulting performance for the inherently more complex, nonlinear task of reaching a desired end-effector position in the face of an obstacle, as illustrated in \figref{fig:title_hw_apollo}. Now, it is not sufficient to simply drive the end-effector in the direction of the reference. Instead, multiple changes of direction are necessary to avoid the obstacle.

The state available to the agent is the same as introduced in \secref{sec:apollo_setup_definition}. Thus, the learning agent is only aware of the end-effector position $x_\text{ef}$ in task space. The algorithm's goal is to reach the desired reference position $x_\text{ref}$ without hitting the obstacle with the end-effector. We assume a static obstacle position, as otherwise, this information would need to be provided to the agent. The reference position is now defined in software and not retrieved via the Vicon system. 

We adapt the previously presented training procedure as follows. The starting and reference positions are sampled from the intervals 
%$\begin{pmatrix} [0.45, 0.55] & [0.7, 0.9] & [0.0, 0.2] \end{pmatrix}^\transp \SI{}{\meter}$,
$([0.45, 0.55],~[0.7, 0.9],~[0.0, 0.2])^\transp \SI{}{\meter}$, 
and 
%$\begin{pmatrix} [-0.2, -0.1] & [0.7, 0.9] & [-0.1, 0.1] \end{pmatrix}^\transp \SI{}{\meter}$, 
$([-0.2, -0.1],~[0.7, 0.9],~[-0.1, 0.1])^\transp \SI{}{\meter}$,
respectively. This way, they are separated, with the obstacle in between at 
%$\begin{pmatrix} [-0.05, 0.35] & [0.5, 1.0] & [-1.0, 0.1] \end{pmatrix}^\transp \SI{}{\meter}$. 
$([-0.05, 0.35],~[0.5, 1.0],~[-1.0, 0.1])^\transp \SI{}{\meter}$.
Moreover, during training only, before applying the control action to the system, we predict the next position of the end-effector using integrator dynamics, \ie $x_\text{pred,ef}[k+1]=x_\text{ef}[k]+\Delta T u_\text{ac}[k]$. If the next predicted position $x_\text{pred,ef}[k+1]$ lies inside the obstacle, we apply 
%$u_\text{ac}[k]= \begin{pmatrix} 0 & 0 & 0 \end{pmatrix}^\transp$
$u_\text{ac}[k]= (0,~0,~0)^\transp$ 
to the system, and additionally penalize this state/action combination in the reward function. Thus, the reward is now given by $R = \sum_{k=0}^N \gamma^k (R_{\text{ctrl}}[k] + R_{\text{comm}}[k] + R_{\text{obst}}[k]) = \sum_{k=0}^N \gamma^k (-3(0.01 {\norm{u[k]}_2}^2 + 10 {\norm{x_{\text{ref}}[k] - x_{\text{ef}}[k]}_2}^2 + 0.01 {\norm{\dot{x}_\text{ef}[k]}_2}^2   + \lambda \delta[k]) + \frac{5}{{\norm{x_{\text{ref}}[k] - x_{\text{ef}}[k]}_2}^2} - \zeta[k])$, where
\begin{equation*}
\zeta[k] = \begin{cases} 0, & \text{if } x_\text{pred,ef}[k+1] \text{ not inside obstacle area} \\
5, & \text{otherwise.}
\end{cases}
\end{equation*}
For obtaining the results presented in \figref{fig:hw_rollout_obst}, we first pretrain the policy for 2250 epochs in simulation and then evaluate it on the real hardware.

As shown in \figref{fig:hw_rollout_obst}, \figref{fig:title_hw_apollo}, and the associated video, the reference position is reached reliably without hitting the obstacle, while still \SI{92}{\percent} of communication can be saved. This behavior is consistent among different starting and reference positions. However, compared to the previously presented reference tracking, without the obstacle present, the reference position is not reached as accurately. The reason for this behavior is that the presence of the obstacle limits the freedom of the arm and the policy, resulting in less accuracy. The fact that the reference position is now defined in software and not noisy could explain why more communication can be saved compared to the previously presented dynamic cup reaching scenario (\secref{sec:dynamic_reaching}).
%\footnote{\url{https://youtu.be/NwwV5uxj9bg}}

\begin{figure}
\centering
\includegraphics[height=0.9\textheight,keepaspectratio,width=\collen]{img/HW/obst/final_obst.eps}
\caption{Exemplary obstacle avoidance trajectory, where a fixed reference position is to be reached in the face of an obstacle, cf. \figref{fig:title_hw_apollo}. During the rollout, the policy saves \SI{92}{\percent} of communication, while the reference is reached reliably without hitting the obstacle. This performance is consistent among various runs.}
\label{fig:hw_rollout_obst}
\end{figure}
%Video available at \protect\url{https://youtu.be/NwwV5uxj9bg}.

==> chapters_old/8_TowardsStabilityChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section{Towards Stability of Event-triggered Control}
\label{sec:stability_statment}

In the previous sections, we tackle the \gls{etc} problem formulation using model-free, deep \gls{rl}. The results of our learning algorithm are \gls{nn} policies consisting of many parameters. In this setting, it is usually difficult to provide stability guarantees. Yet, since the learned policies are also envisioned to be used in real-world scenarios, such guarantees are essential. In the following, we present an approach toward checking the stability of learned \gls{nn} policies.
As a starting point, in this work, we restrict to \glspl{nn} parametrized with \glspl{relu}, and known, linear system dynamics.
%\nf{enough to allude why called towards or shall we add sclability issue,... I think main point why calling TOWARD: model-free rl and model-based verification,...} 
%\st{This will be a bit tricky, but I think the intro paragraph should also allude to why we call this "Toward".  That is, what does the following provide/contribute, but what are the (current) limitations.  For example, one could say that the stability analysis holds for the proposed method as long as you use ReLU and the networks aren't too large?  The reader should undestand the scope of whta is coming.}

\subsection{Stability Verification of Neural Network Policies}
\label{sec:stabi_veri_nn}

The following stability analysis is based on the Marabou framework proposed in~\cite{katz2017reluplex,katz2019marabou}, which allows to check for properties of deep \glspl{nn}. The Marabou framework is an expansion of the Simplex method \cite{dantziglinear}. Simplex tries to find a valid assignment to a linear program. It either returns an admissible value for all the free variables involved that result in satisfying the query, or returns that the query is not satisfiable. As piecewise linear activation functions can be interpreted as case dependent linear constraints, the authors expand the algorithm such that the same satisfiability queries, as for the Simplex method, can be posed with respect to \glspl{nn}.

We exploit this framework to come up with stability guarantees for trained policies. For our considerations, the only limitation is that exclusively piecewise linear activation functions, \ie \gls{relu} activations can be used within the networks. Nevertheless, by combining the algorithm with assumptions on the system dynamics, it is possible to provide stability guarantees through output range analysis for the learned \gls{nn} policies.
Further, in case the policy does not fulfill the stability requirements straight away, the framework can be used to develop a retraining procedure to refine the \glspl{nn}. 

% Further, the properties of the framework, \ie returning a valid assignment to a query, if available, helps to develop a retraining procedure to refine the \glspl{nn} in case that the desired stability statements are not fulfilled straight away.


\subsection{Stability Analysis and Retraining of Event-triggered Control Policies}

We define stability as finding a positive invariant set in the state space: once inside this set, when applying the \gls{nn} policy, the next state is guaranteed to also lie within this set. 

\begin{defi}[Stability]{$\text{ }$\\}
The system $f$ is considered stable under the \gls{nn} control policy~$u_\text{NN}[k]=h_\text{NN}(\tilde{x}[k])$ if there exists a region $\mathcal{O}$, such that \\
$x[k] \in \mathcal{O} \Rightarrow x[k+1]\!=\!f(x[k],h_\text{NN}(\tilde{x}[k])) \in  \mathcal{O} \text{ } \forall x[k] \in\mathcal{O}$.
\label{def:stability_def}
\end{defi}

While the \gls{rl} algorithm presented in \algref{alg:learn_etc} is model-free and can be used for systems with linear or nonlinear dynamics, the stability check relies on the underlying system exhibiting known, linear dynamics. The algorithm then checks whether the control policy is stable, according to \defref{def:stability_def}. Linear system dynamics can also be represented using \glspl{relu}. Thus, algorithmically, we can design one \gls{nn} that takes as the input the current state $x[k]$ and outputs the next state $x[k+1]$, \cf \figref{fig:MarabouSchematicET}. With this network given, we can exploit the Marabou framework \cite{katz2019marabou} to check for the desired properties. 

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=1.0\collen]{img/Marabou/schematic/Marabou.png}
\caption{Schematic of the pipeline used for the stability verification. The parts inside the blue box can all be parametrized using \gls{relu} units. Therefore, the algorithm can check whether the next state is inside the same set as the current state. This is the basis for our stability analysis.}
\label{fig:MarabouSchematic}
\end{figure}
\end{comment}

\subsubsection{Stability Analysis of the Policies}

\begin{figure}
\centering
%\includegraphics[width=1.0\collen]{img/Marabou/schematic/ET.png}
\includegraphics[width=1.0\collen]{img/Marabou/schematic/InputCheckET_new.pdf}
\caption{Schematic of the pipeline used for the stability verification procedure. The parts inside the blue box can all be parametrized using \gls{relu} units. Therefore, the Marabou framework can check whether the next state is inside the same set as the initial state. This is the basis for our stability analysis.}
\label{fig:MarabouSchematicET}
\end{figure}
%\st{I don't like the rendering of the block diagrams.  I suggest having the same line width and font size for all block diagrams.  Arrow-heads could be slightly larger.  Also, I would not use red color for the outer box.}

In the \gls{et} setting, the next state depends on the communication decision. Therefore, effectively two next states have to be calculated, as shown in \figref{fig:MarabouSchematicET}. 
To make use of the deterministic Marabou framework, we need to eliminate the stochasticity of the communication decision.
Hence, we always choose to communicate in case the probability is larger than or equal to \SI{50}{\percent}.
% To make use of the deterministic Marabou framework, the stochasticity of the communication decision is eliminated. Whenever the probability for communication is larger than or equal to \SI{50}{\percent}, this decision is taken and vice versa. 


The resulting algorithm that checks for the stability of a region $\mathcal{O}$ is presented in \algref{alg:check_stab_et}. As the input to the stability verification framework (see \figref{fig:MarabouSchematicET}) is given by $\tilde{x}[k]$, we additionally define 
%$\mathcal{S} = \begin{pmatrix} \mathcal{O} & \mathcal{L} \end{pmatrix}^\transp = \begin{pmatrix} \mathcal{O} & [-u_\text{lim},u_\text{lim}] \end{pmatrix}^\transp$,
$\mathcal{S} = (\mathcal{O},~\mathcal{L})^\transp = (\mathcal{O},~[-u_\text{lim},u_\text{lim}])^\transp$, 
which combines the stable region with the input range. Adding the input range is necessary as it covers the potential range of the previously applied control actions, which are reapplied in case the \gls{zoh} is selected. If the algorithm returns an empty set of points, we know that given the region $\mathcal{O}$, the input range, and the system dynamics, the \gls{etc} policy is stable. Otherwise, the algorithm directly outputs exemplary unstable points $\tilde{x}[k]$.  %for which, after applying the \gls{etc} strategy, the next state lies outside the invariant set.
There are two possibilities, why a point $\tilde{x}[k]$ is unstable under the \gls{etc} policy. Either the policy erroneously decides to skip communication, and the reapplication of the previous control input results in the next state outside the invariant set. Or, in case of communication, the policy chooses an unstable control input.

%We present an algorithm (\algref{alg:check_stab_et}) that checks for the stability of a two-dimensional system. In this setting, the stable region is given by $\mathcal{O}= \begin{pmatrix} [x_{1,\text{l}},x_{1,\text{h}}] & [x_{2,\text{l}},x_{2,\text{h}}] \end{pmatrix}^\transp$. As the input to the checking framework is given by $\tilde{x}[k]$, we additionally define $\mathcal{S} = \begin{pmatrix} \mathcal{O} & \mathcal{L} \end{pmatrix}^\transp = \begin{pmatrix} \mathcal{O} & [-u_\text{lim},u_\text{lim}] \end{pmatrix}^\transp$. To guarantee stability for this region, we have to check for the stability of every bounding edge separately. That is why the \textit{CheckIntervalET} function is called 4 times.
%\db{the 2-dimensional example is nice, but since we don't really use it I would leave it out. I agree, I will think about how to make this shorter.}

%Focussing on the general idea only and neglecting the low-level implementation, \algref{alg:check_stability_ET_rigorous} can be rewritten for arbitrary dimensions, as shown in \algref{alg:check_stab_et}. If the algorithm returns an empty set of points, we know that given the region $\mathcal{O}$ and the dynamics of the system, our \gls{nn} control policy is stable. Otherwise, the algorithm directly outputs exemplary points $\tilde{x}[k]$, for which, after applying the \gls{nn} control policy, the next state lies outside the stable region.

\begin{comment}
\begin{algorithm}
\caption{Check for Stability of $\mathcal{S}$ in ETC, exemplarily for $\mathbb{R}^2$}
\label{alg:check_stability_ET_rigorous}
\begin{algorithmic}[1]
  \scriptsize
  \item[]
	\Function{CheckIntervalET}{$\Phi$} \label{line:start_checkinterval_et} 
	\State points=$[]$
  	\State query to Marabou: $\tilde{x}[k] \in \mathcal{S} \Rightarrow x_{\delta=0}[k+1] \in  \Phi \text{ for } P(\delta[k]=1)<0.5$ \label{line:start_sav_comm_et}
  	\If {Valid assignment is found:}
  		\State points.append($\tilde{x}[k]$)
  	\EndIf \label{line:end_sav_comm_et}
  	\State query to Marabou: $\tilde{x}[k] \in \mathcal{S} \Rightarrow x_{\delta=1}[k+1] \in  \Phi \text{ for } P(\delta[k]=1) \geq 0.5$ \label{line:start_communicate_et}
  	\If {Valid assignment is found:}
  		\State points.append($\tilde{x}[k]$)
  	\EndIf \label{line:end_communicate_et}
  	\State \Return points
  \EndFunction \label{line:end_checkinterval_et}
  \item[]
  
   \State $\mathcal{O} = \begin{pmatrix} 	[x_{1,\text{l}},x_{1,\text{h}}] \\ [x_{2,\text{l}},x_{2,\text{h}}] \end{pmatrix}$
   \item[]
  \State $\mathcal{S} = \begin{pmatrix} 	\mathcal{O} \\ [-u_\text{lim},u_\text{lim}] \end{pmatrix}$
  \item[]
  \State points=$[]$
  \State points.append(\Call{CheckIntervalET}{$\Phi=\begin{pmatrix}
  (-\infty,x_{1,\text{l}}) \\ (-\infty,\infty) \end{pmatrix}$})
  \State points.append(\Call{CheckIntervalET}{$\Phi=\begin{pmatrix}
  (x_{1,\text{h}},\infty) \\ (-\infty,\infty) \end{pmatrix}$})
  \State points.append(\Call{CheckIntervalET}{$\Phi=\begin{pmatrix}
  (-\infty,\infty) \\ (-\infty,x_{2,\text{l}}) \end{pmatrix}$})
  \State points.append(\Call{CheckIntervalET}{$\Phi=\begin{pmatrix}
  (-\infty,\infty) \\ (x_{2,\text{h}},\infty) \end{pmatrix}$})
  \State \Return points
\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{algorithm}
\caption{Check for Stability in ET setting ($\mathcal{S}$)}
\label{alg:check_stab_et}
\begin{algorithmic}[1]
  \scriptsize
  \State points=$[]$
  \State Marabou query: $\tilde{x}[k] \in \mathcal{S} \text{, } P(\delta[k]=1)\geq 0.5 \Rightarrow x_{\delta=1}[k+1] \in  \mathbb{R}^{n} \setminus \mathcal{O}$
  \If {Valid assignment is found:} {points.append($\tilde{x}[k]$)} \EndIf
   \State Marabou query: $\tilde{x}[k] \in \mathcal{S} \text{, } P(\delta[k]=1) < 0.5 \Rightarrow x_{\delta=0}[k+1] \in  \mathbb{R}^{n} \setminus \mathcal{O}$
  \If {Valid assignment is found:} {points.append($\tilde{x}[k]$)} 
  \EndIf
  \State \textbf{return} points
\end{algorithmic}
\end{algorithm}



\subsubsection{Retraining Neural Network Policies}


If \algref{alg:check_stab_et} does not indicate stability, \ie returns a non-empty set of points, it is possible to refine the \gls{etc} policy such that it fulfills the invariance property using \algref{alg:refine_pol ET}.

At the core of this algorithm is the \textit{FindValidInputET} function (ll.~\ref{line:start_validinput_et}-\ref{line:end_validinput_et}). In case the stability verification algorithm (\algref{alg:check_stab_et}) returns an unstable point, we feed it into the schematic presented in \figref{fig:InputCheckSchematic} and Marabou returns a value for the input $u[k]$ such that the next state $x[k+1]$ also lies inside the invariant set.

\begin{figure}
\centering
%\includegraphics[width=0.66\collen]{img/Marabou/schematic/InputCheck.png}
\includegraphics[width=0.6756\collen]{img/Marabou/schematic/InputCheck_new.pdf}
\caption{Schematic of the pipeline that is used to find an admissible input $u[k]$ for an unstable point $x[k]$. The parts inside the blue box can all be parametrized using \gls{relu} units.}
\label{fig:InputCheckSchematic}
\end{figure}

In case a point $\tilde{x}[k]$ is unstable using the current policy, both parts of the \gls{et} controller have to be adapted. On the one hand, it is crucial to ensure that an appropriate control action is chosen. On the other hand, we have to ensure that the policy decides to communicate. This supervised retraining for unstable points can be seen in ll.~\ref{line:start_supervised-line}-\ref{line:end_supervised-line} of \algref{alg:refine_pol ET}. We define that at those points, the probability of communication should be set to \SI{60}{\percent}. Note that any choice above \SI{50}{\percent} is admissible.

When using the previously described mechanism, all the refined policies exhibit significantly reduced communication savings as any unstable configuration can only be resolved using communication. Thus, we found it beneficial to sample additional points using Sobol sequences \cite{sobol1976uniformly} to cover the whole state space as thoroughly as possible (l.~\ref{line:sobol_samp} of \algref{alg:refine_pol ET}). We then add the condition to the retraining procedure that communication must be saved whenever possible (ll.~\ref{line:start_commsav_et}-\ref{line:end_commsav_et} and \ref{line:start_supervised_enforce-line}-\ref{line:end_supervised_enforce-line}). This can also be interpreted as trying to be maximally resource-efficient.

Combining the individual parts results in \algref{alg:refine_pol ET}. 
% This algorithm is capable of retraining policies. 
If the algorithm terminates, we know that the \gls{etc} law is stable for the defined region $\mathcal{O}$, the input range, and the assumed system dynamics.

\begin{algorithm}
\caption{Refine Policy ET}
\label{alg:refine_pol ET}
\begin{algorithmic}[1]
  \scriptsize

  %\item[]
  \Function{FindValidInputET}{$\tilde{x}[k],\mathcal{O}$}  \label{line:start_validinput_et}
	%\Comment{Recall $\tilde{x}[k]=\begin{pmatrix} x[k] & u[k-1] \end{pmatrix}^\transp$.}
	\State Marabou query: $\text{find } u[k] \text{, s.t. } x[k], u[k] \Rightarrow x[k+1] \in \mathcal{O}$	  	
  	\State \Return $u[k]$
  \EndFunction \label{line:end_validinput_et}
  \item[]


  \Function{CheckPointET}{$\tilde{x}[k],\mathcal{O}$} \label{line:start_checkpoint_et}
	\State points=$[]$
	\State Marabou query: $\tilde{x}[k] \Rightarrow x[k+1] \in  \mathbb{R}^{n} \setminus \mathcal{O}$ 
  \If {Valid assignment is found:} {points.append($\tilde{x}[k]$)} 
  \EndIf
  \State \textbf{return} points
  \EndFunction \label{line:end_checkpoint_et}
  \item[]
  
  \Function{CommSavingPossible}{$\tilde{x}[k],\mathcal{O}$}  \label{line:start_commsav_et}
  	\State points=$[]$
  	\Comment{Check whether next state is also stable without communicating.}
  	\State Marabou query: $\tilde{x}[k] \Rightarrow x_{\delta=0}[k+1] \in  \mathcal{O} \text{ for } P(\delta[k]=1)$ $\geq 0.5$
  	\If {Valid assignment is found:} {points.append($\tilde{x}[k]$)} 
  	\EndIf
	\State \Return points
  \EndFunction \label{line:end_commsav_et}
  \item[]    
  
  \State Choose region $\mathcal{O}$
  \State Define region $\mathcal{S} = (\mathcal{O},~[-u_\text{lim},u_\text{lim}])^\transp$
  \State $\text{points}_\text{crit}$ $=$ Check for Stability ($\mathcal{S}$), see \algref{alg:check_stab_et}
  \While {not $\text{points}_\text{crit}$ is EMPTY}
	\Comment{Use Sobol sequences to generate additional points}
	\State $\text{points}_\text{sobol}$ $=$ Use sobol sequence to sample from $\mathcal{S}$ \label{line:sobol_samp}
    \State $\text{points}_\text{commsav} = []$
    \For {$\tilde{x}[i]$ in $\text{points}_\text{sobol}$ }
  		\State $\text{points}_\text{crit}$.append(\Call{CheckPointET}{$\tilde{x}[i],\mathcal{O}$}
  		\State $\text{points}_\text{commsav}$.append(\Call{CommSavingPossible}{$\tilde{x}[i],\mathcal{O}$}
  	\EndFor  
  	\Comment{Calculate admissible input for all the unstable points.}
	\State $u_\text{crit}=[]$  	
  	\For {$\tilde{x}[i]$ in $\text{points}_\text{crit}$}
  		\State $u_\text{crit}$.append(\Call{FindValidInputET}{$\tilde{x}[i],\mathcal{O}$}
  	\EndFor
  	\Comment{Supervised retraining to enforce communication savings}
  	\For {number of optimizer epochs} \label{line:start_supervised_enforce-line}
  		\State $L_2(\theta_2)=(P(\delta[k]=1|\text{points}_\text{commsav},\theta_2) - 0.4)^2$
  		\State $\theta_2 = \theta_2 - \alpha_{\theta_2} \frac{\partial L_2}{\partial \theta_2}$
  	\EndFor \label{line:end_supervised_enforce-line}
  	\Comment{Supervised retraining of the NN policy for critical points}
  	\For {number of optimizer epochs} \label{line:start_supervised-line}
  		\State $L_1(\theta_1)=(u_\text{NN}(\text{points}_\text{crit},\theta_1)-u_\text{crit})^2$
  		\State $L_2(\theta_2)=(P(\delta[k]=1|\text{points}_\text{crit},\theta_2) - 0.6)^2$
  		\State $\theta_1 = \theta_1 - \alpha_{\theta_1} \frac{\partial L_1}{\partial \theta_1}$
  		\State $\theta_2 = \theta_2 - \alpha_{\theta_2} \frac{\partial L_2}{\partial \theta_2}$
  	\EndFor \label{line:end_supervised-line}
  \State $\text{points}_\text{crit}$ $=$ Check for Stability ($\mathcal{S}$), see \algref{alg:check_stab_et}
  \EndWhile
\end{algorithmic}
\end{algorithm}


\subsection{Simulation Example}

In the following section, we demonstrate the previously presented algorithm. The task is to obtain a guaranteed stable \gls{et} controller for stabilizing the inverted pendulum on top in the OpenAI Gym Pendulum environment. We use the exact same configuration as in \secref{sec:poc}. In line with Definition \ref{def:stability_def}, we define the safe state space ($\mathcal{O}$) to capture ranges of $\theta \in [\SI{-2.5}{\degree},\SI{2.5}{\degree}]$ and $\dot{\theta} \in [\SI{-5}{\degree / \second},\SI{5}{\degree / \second}]$.  Usually, the state of the pendulum environment that is fed into the \glspl{nn} is given by 
%$x[k]=\begin{pmatrix} \cos(\theta[k]) & \sin(\theta[k]) & \dot{\theta}[k] \end{pmatrix}^\transp$.
$x[k]=(\cos(\theta[k]),~\sin(\theta[k]),~\dot{\theta}[k])^\transp$. 
However, for the stability verification algorithm, we need to express the \gls{nn} policies' output in terms of the system variables, \ie $\theta[k]$ and $\dot{\theta}[k]$. Thus, we can neither use the nonlinear sine nor the cosine function and linearize the state of the environment around the equilibrium, which results in 
%$x[k] \approx \begin{pmatrix} 1.0 & \theta[k] & \dot{\theta}[k] \end{pmatrix}^\transp$.
$x[k] \approx (1.0,~\theta[k],~\dot{\theta}[k])^\transp$.

The results of running the retraining procedure (\algref{alg:refine_pol ET}) are shown in \figref{fig:retrain_et_pendulum}. We initialize the procedure with a policy that has been trained for 500 epochs using our proposed training algorithm (\algref{alg:learn_etc}). As can be seen in \figref{fig:retrain_et_pendulum_unstable}, this policy is not stable yet. Running the retraining procedure for 4 epochs results in a guaranteed stable \gls{et} controller that keeps the pendulum upright (see \figref{fig:retrain_et_pendulum_stable}). Although we only trained for an angular region between \SI{-2.5}{\degree} and \SI{2.5}{\degree}, the policy also yields a stabilizing performance when starting outside of this interval, as shown in \figref{fig:retrain_et_pendulum_stable}. Over 10 randomly started runs, the policy saves around \SI{70}{\percent} of communication. An exemplary rollout of this very resource-efficient and guaranteed stable control policy is presented in \figref{fig:retrain_et_pendulum_rollout}.

%So far, attempts to apply the herein presented results onto higher dimensional environments have been unsuccessful, since the complexity for checking larger \glspl{nn} or higher dimensional systems quickly increases. We nevertheless hope that advances in computational power as well as progress in the underlying verification algorithms will enable to scale the ideas in the future. \nf{not sure if this is a good reasoning why we cannot scale to higher dimensions,...} 
%\db{I would leave this out here and discuss it in the conclusions. Also don't need to go into too much detail, just saying that scaling to higher dimensional systems is an issue because computational complexity increases is enough.}

\begin{figure}
\begin{subfigure}{1.0\collen}
	\centering
	\begin{subfigure}[t]{0.5225\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/full/before.eps}
	\caption{Exemplary rollouts for trying to stabilize a pendulum with an \gls{et} policy, which has been trained for 500 optimization epochs. This policy does not succeed in keeping the pendulum upright.}
	\label{fig:retrain_et_pendulum_unstable}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.4275\textwidth}
	\includegraphics[width=\textwidth]{img/Marabou/full/after.eps}
	\caption{Exemplary rollouts for stabilizing a pendulum after retraining the policy from \figref{fig:retrain_et_pendulum_unstable} with \algref{alg:refine_pol ET} for 4 epochs. This policy is guaranteed to stabilize the pendulum on top.}
	\label{fig:retrain_et_pendulum_stable}
	\end{subfigure}
\end{subfigure}
\caption{Effect of the retraining procedure presented in \algref{alg:refine_pol ET}. In the plots, each color represents a different rollout. While the initial policy is unstable (\figref{fig:retrain_et_pendulum_unstable}), after refining this policy for 4 iterations using \algref{alg:refine_pol ET}, a guaranteed stable controller is obtained which successfully stabilizes the pendulum and still saves about \SI{70}{\percent} of communication (\figref{fig:retrain_et_pendulum_stable}).}
\label{fig:retrain_et_pendulum}
\end{figure}
% Additional rollout I think not needed:
%\begin{comment}
\begin{figure}
\centering
\includegraphics[width=1.0\collen]{img/Marabou/full/ex_rollout.eps}
\caption{Illustration of an exemplary rollout of the same policy as shown in \figref{fig:retrain_et_pendulum_stable}.}
\label{fig:retrain_et_pendulum_rollout}
\end{figure}
%\end{comment}




























% Is left here but not needed:
\begin{comment}

\subsubsection{Retraining Neural Network Policies - Periodic Control}
\label{sec:retrain_periodic}

If \algref{alg:check_stab} does not indicate stability, \ie returns a non-empty set of points, it is possible to refine the \gls{nn} policy such that it fulfills the desired property, using \algref{alg:refine_pol}.

At the core of this algorithm is the \textit{FindValidInput} function, which is introduced in lines~\ref{alg:validinputstart-line} - \ref{alg:validinputend-line}. This function exploits the fact that the framework tries to assign admissible values to the free variables to satisfy the query. Therefore, if the stability checking algorithm returns a point where the \gls{nn} controller results in an unstable input, we feed this point into the schematic presented in \figref{fig:InputCheckSchematic} and Marabou returns a value for the input $u[k]$ such that the next state $x[k+1]$ also lies within the stable set. We can then use those samples consisting of the state $x[k]$ and admissible input $u[k]$ to update the parameters $\theta$, of the \gls{nn} policy, using gradient descent, as shown in lines ~\ref{alg:supervisedstart-line} - \ref{alg:supervisedend-line} of \algref{alg:refine_pol}, where $u_\text{NN}$ denotes the output of the \gls{nn} policy.

\begin{figure}
\centering
\includegraphics[width=1.0\collen]{img/Marabou/schematic/InputCheck.eps}
\caption{Schematic of the pipeline used for finding an admissible input $u[k]$ for an unstable point $x[k]$. The parts inside the blue box can all be parametrized using \gls{relu} units.}
\label{fig:InputCheckSchematic}
\end{figure}

\begin{algorithm}
\caption{Refine Policy}
\label{alg:refine_pol}
\begin{algorithmic}[1]
  \scriptsize

  \item[]
  \Function{FindValidInput}{$x[k],\mathcal{O}$}  \label{alg:validinputstart-line}
  	\State \Return $u[k] \text{, s.t. } x[k], u[k] \Rightarrow x[k+1] \in \mathcal{O}$
  \EndFunction \label{alg:validinputend-line}
  \item[]  
  
  \State Choose region $\mathcal{O}$
  \State points $=$ Check for Stability ($\mathcal{O}$), see \algref{alg:check_stab}
  \While {not points is EMPTY}
	\State $u=[]$  	
  	\For {$x[i]$ in points}
  		\State $u$.append(\Call{FindValidInput}{$x[i],\mathcal{O}$}
  	\EndFor
  	\State \Comment{Supervised retraining of the NN policy $u_\text{NN}$}
  	\For {number of optimizer epochs} \label{alg:supervisedstart-line}
  		\State $L(\theta)=(u_\text{NN}(\theta,\text{points})-u)^2$
  		\State $\theta = \theta - \alpha_\theta \frac{\partial L}{\partial \theta}$
  	\EndFor \label{alg:supervisedend-line}
  \State points $=$ Check for Stability ($\mathcal{O}$), see \algref{alg:check_stab}
  \EndWhile
\end{algorithmic}
\end{algorithm}

In theory, \algref{alg:refine_pol} is sufficient to refine the policy. However, as \algref{alg:check_stab} only returns exemplary unstable points, we found it beneficial to sample additional points using Sobol sequences \cite{sobol1976uniformly}. For those points, we also check whether the \gls{nn} policy chooses an appropriate input such that the next state is stable. If this check fails, those points are also added to the supervised retraining. The additional sampling stabilizes the process, as it ensures better coverage of the state space. Note that the retraining only uses the points where the \gls{nn} outputs an unstable control action.


\begin{remark}
As this framework is currently limited to linear system dynamics, we propose the following modification for nonlinear systems. Instead of directly inserting the system dynamics, the goal would be to approximate the nonlinear dynamics using \gls{relu} units and to then insert this block into the schematic in \figref{fig:MarabouSchematic} and use the original algorithm.
\end{remark}

\end{comment}


==> chapters_old/9_DiscussionOutlookChapter.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../learning_et_ctrl.tex

\section{Conclusion}
\label{chp:Conclusion_and_Outlook}

In this paper, we propose a model-free hierarchical \gls{rl} algorithm capable of jointly learning event-triggered control policies from scratch. %for a wide range of environments. %The algorithm is mainly based on the ideas presented in \cite{OptionCriticContPaper}, which have been adapted and expanded considerably to arrive at the presented results.
%While the algorithm is capable of learning \gls{etc} in linear environments\db{leave out}, the main novelty lies in the fact that it also scales to high-dimensional, nonlinear, and very complex simulation environments, without any modifications.
Without any modification, the algorithm can be applied to linear and nonlinear, low- and high-dimensional systems.
In those high-dimensional environments, communication savings of up to \SI{80}{\percent} can be reported. To the best of our knowledge, our algorithm is the first that can obtain event-triggered policies for such environments through joint optimization.

The algorithm is also successfully deployed on real hardware, \ie the Apollo robot. We provide a demonstration for resource-efficient setpoint tracking and obstacle avoidance while saving around \SI{85}{\percent} and \SI{90}{\percent} of communication, respectively. These results imply that the presented algorithm scales to partially observable settings, to using more than 2 options, and to imperfect communication settings with potential delays.

Moreover, we show a novel algorithm for evaluating the stability of linear systems controlled by \gls{nn} policies. In case the learned \gls{et} policy initially does not yield the desired stability guarantee, we propose a retraining procedure for refining the previously unstable policy. 
%Those results mainly rely on extensions of the work by Katz et al. \cite{katz2017reluplex,katz2019marabou}. 
Scaling those ideas to nonlinear environments, as well as higher-dimensional systems through handling the increased computational complexity, is subject to ongoing research.
%Ongoing research currently investigates how to scale those ideas to higher-dimensional systems as the computational complexity quickly increases. Expanding the algorithms to nonlinear environments is another direction worthwhile investigating.
% is an issue because the computational complexity quickly increases. \st{So, scalability is the main limiting factor of our verification, right?  Don't just say that it is an issue (don't be too negative); could mention that this is a topic of ongoing research.}

%Additional ideas for future work include extending the results presented herein to multi-agent scenarios and settings with imperfect communication, \ie message loss. Lastly, an attempt to further increase resource-efficiency would be to explore adding ideas from self-triggering, and, therefore, also actively trying to save communication between the sensors and the agent.
%\db{This part I would leave out and I would also call this section Conclusion only}



%\db{I would write this from a more positive viewpoint. Something like interesting ideas for future work considerations include extending the results presented herein to multi-agent scenarios and settings with imperfect communication, \ie message loss and delays.

%Moreover, expanding the stability verification and retraining procedure to nonlinear and more high-dimensional environments is another direction worthwhile investigating.
%Also, this part doesn't need to be super long.}


%In this work, we considered learning \gls{etc} strategies from data for single-agent scenarios. Further, we assume perfect conditions, \ie no delays, package losses, or additional disturbances due to the communication involved. Additionally, our stability verification and retraining procedure is currently limited to linear system dynamics. 

%One consideration of future work would be to expand the ideas and to make use of them in multi-agent scenarios. Adding more agents to the system naturally increases the risk of package losses or delays. It would, therefore, be necessary to include those imperfections in the problem formulation and stability verification procedure. The stability verification algorithm should also be expanded to arrive at robustness statements and to scale to nonlinear system dynamics. Ultimately, the model underlying the stability statements should also be actively learned from data and the verification procedure should be incorporated more closely into the learning process. To further increase the resource-efficiency of the overall approach, it would be interesting to investigate adding ideas from self-triggering. While the current framework only considers saving communication between the agent and the actuator, those concepts also address the link between the sensors and the agent, therefore, holding great potential for even higher energy and communication savings.
